A Comprehensive Review of Automated Data Annotation Techniques in Human Activity Recognition

Human Activity Recognition (HAR) has become one of the leading research topics of the last decade. As sensing technologies have matured and their economic costs have declined, a host of novel applications, e.g., in healthcare, industry, sports, and daily life activities have become popular. The design of HAR systems requires different time-consuming processing steps, such as data collection, annotation, and model training and optimization. In particular, data annotation represents the most labor-intensive and cumbersome step in HAR, since it requires extensive and detailed manual work from human annotators. Therefore, different methodologies concerning the automation of the annotation procedure in HAR have been proposed. The annotation problem occurs in different notions and scenarios, which all require individual solutions. In this paper, we provide the first systematic review on data annotation techniques for HAR. By grouping existing approaches into classes and providing a taxonomy, our goal is to support the decision on which techniques can be beneficially used in a given scenario.

==> authors/cristian_bib.tex <==
 % !TEX root = ../main.tex

 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.1in,clip]{authors/cristian.jpeg}}]
    {\textbf{Cristian Turetta}} received the B.S. and M.E. degrees in Computer Science and Engineering from the University of Verona, Italy, respectively in 2017 and 2020. 
    He is currently a PhD student at the Department of Computer Science of the University of Verona, where he is a member of the IoT4care research group working on Ambient Assisted Living and Internet of Things.
\end{IEEEbiography}

==> authors/fadi_bib.tex <==
\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{authors/fadi.png}}]
    {\textbf{Fadi Al Machot}} received the German Diploma degree in computer science from the University of Potsdam, in 2010, the Ph.D. degree
in computer science from Klagenfurt University, Austria, in 2013, and the Habilitation degree in applied computer science from the University
of Lübeck, Germany, in 2020. He is currently working as an Associate Professor in machine learning (ML) at the Norwegian University of
Life Sciences (NMBU), Norway. His work has been patented and published in peer-reviewed international conferences and journals. His research interests include deep learning, neural-symbolic learning, video understanding, cognitive modeling, and zero/few-shot learning.
\end{IEEEbiography}

==> authors/florenc_bib.tex <==
% !TEX root = ../main.tex
\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{authors/florenc.jpg}}]{\textbf{Florenc Demrozi,}} PhD in computer science, IEEE member, IFIP WG 10.5 member, received the B.S. and M.E. degrees in Computer Science and Engineering from the University of Verona, Italy, respectively in 2014 and 2016, and the Ph.D. degree in Computer Science from University of Verona, Italy, in 2020. He is currently an Associate Professor in Biomedical Engineering at the Department of Electrical Engineering and Computer Science, University of Stavanger, Norway, working on Human Activity Recognition (HAR), Ambient Assisted Living (AAL), Internet of Medical Things (IoMT), Sensors and Measurements. 
\end{IEEEbiography}

==> authors/graziano_bib.tex <==
% !TEX root = ../main.tex

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{authors/graziano.jpg}}]
    {\textbf{Graziano Pravadelli,}} PhD in Computer Science, IEEE senior member, IFIP 10.5 WG member, is full professor of information processing systems at the Computer Science Department of the University of Verona (Italy) since 2018, where he lead the IoT4care research group. 
    In 2007 he cofounded EDALab s.r.l., an SME working on the design of IoT-based monitoring systems. 
    His main interests focus on system-level modeling, simulation and semi-formal verification of embedded systems, as well as on their application to develop IoT-based virtual coaching platforms for people with special needs. 
    In the previous contexts, he collaborated in several national and European projects and he published more than 120 papers in international conferences and journals.
\end{IEEEbiography}

==> authors/kindt_bib.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.25in,clip,keepaspectratio]{authors/Philipp-Kindt.jpg}}]
    {\textbf{Philipp H. Kindt}} received his Ph.D. in Electrical Engineering from the Technical University of Munich in 2019. He was an assistant professor (“Juniorprofessor”) of pervasive computing systems at the Chemnitz University of Technology, and is currently working in the economy. His research interests are wireless communication, mobile computing and the IoT. 
\end{IEEEbiography}

==> doc/4-meth_old.tex <==
% !TEX root = ../main.tex
\section{Annotation Systems in HAR}\label{sec:meth}
Based on the analysis of the 39 out of 2401 papers identified through our selection criteria procedure, this systematic review will focus solely on semi-automated and fully-automated data annotation techniques and exclude manual techniques, sensor fusion, and crowdsensing. 
The considered techniques will be first categorized into semi-automated and fully-automated ones, and will then be further classified into the following three categories: a) data-driven, b) environment-driven, and c) hybrid. 

\noindent \textbf{Data-driven:} Data-driven techniques leverage the patterns, structures, and characteristics inherent in the data itself to guide the annotation process.\\%The data-driven techniques rely primarily on the characteristics of the data itself, such as clustering or classification algorithms that group similar data points. \\
\noindent \textbf{Environment-driven:} The environment-driven techniques use information about the context and environment in which the data was collected to perform annotation, such as location, time, or features extracted from the environment. \\
\noindent \textbf{Hybrid:} The hybrid techniques combine both data-driven and environment-driven approaches, often using multiple sources of information to achieve more accurate and robust annotation results.\\ 

This taxonomy is shown in Figure \ref{fig:tax_2}, while Table \ref{tab:all-papers} provides an overview of the studies included in the review and categorized using the taxonomy proposed above.
%This taxonomy is shown in Figure \ref{fig:tax_2}.
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\textwidth,page={4}]{img/figures.pdf}
    \caption{Automatic data annotation taxonomy in HAR (1).}
    \label{fig:tax_2}
\end{figure}

%\noindent Complementary, Table \ref{tab:all-papers} provides an overview of the studies included in the review and categorized using the taxonomy proposed above. 
\begin{table}[!ht]
\centering
\caption{Overview of studies included in this reviewed paper grouped by the mentioned taxonomy (\cite{szewcyzk2009annotating} fits into two categories).  }\label{tab:all-papers}
\resizebox{\textwidth}{!}{
\begin{tabular}{|p{2.5cm}|p{2.5cm}|p{2.5cm}||p{2.5cm}|p{2.5cm}|p{1.5cm}|}
\hline
\multicolumn{6}{|c|}{Data annotation techniques in HAR}\\ \hline \hline
\multicolumn{3}{|c||}{Semi-automated} &\multicolumn{3}{c|}{Fully-automated} \\ \hline \hline
Data-Centric&Environment&Hybrid&Data-Centric&Environment&Hybrid\\
based&based&&based&based&\\ \hline
\cite{saeedi2017co} \cite{martindale2018smart} \cite{gan2018automatic} \cite{bota2019semi} \cite{martindale2019hidden} \cite{ponnada2019designing} \cite{faridee2019augtoact} \cite{hossain2019active} \cite{sawano2020annotation} \cite{kwon2020imutube} \cite{avsar2021benchmarking} \cite{korpela2021reducing} \cite{tang2021selfhar} \cite{yhdego2022fall} \cite{mohamed2022har}&

\cite{szewcyzk2009annotating} \cite{subramanya2012recognizing} \cite{woznowski2017talk} \cite{tonkin2018talk} \cite{solis2019human}&

\cite{alam2015mobeacon} \cite{meurisch2015labels} \cite{nino2016scalable} \cite{cruciani2018personalized} \cite{cruz2019semi} \cite{tonkin2019towards}&

\cite{jardim2016automatic} \cite{rokni2018autonomous} \cite{liang2018automatic} \cite{zhang2020deep} \cite{jeng2021wrist} \cite{ullrich2021detection} \cite{ma2021unsupervised} \cite{qi2022dcnn} \cite{lin2022clustering}&

\cite{szewcyzk2009annotating} \cite{loseto2013mining} \cite{al2017annotation} \cite{demrozi2021towards} \cite{dissanayake2021indolabel}&
\\ \hline \hline
Total: 15&Total: 5*&Total: 6&Total: 9&Total: 5*&Total: 0\\
\hline
\end{tabular}}
\end{table}

In the order of their date of publication, this section will provide a comprehensive overview of each paper included in this survey. Additionally, for each category of our taxonomy, a table that summarizes the most important properties of all publications that fall under the corresponding category is provided.
In particular, Tables \ref{tab:S-DD}, \ref{tab:S-ED}, \ref{tab:S-H}, \ref{tab:H-DD}, and \ref{tab:H-ED} contain detailed information on aspects such as the ownership \add{(i.e., authors used an open access existing dataset or designed and collected new data on their own)} of the tested datasets and the number of datasets utilized (Column 2), the devices (Column 3) and sensors employed (Column 4), the total number of sensors used (Column 5), their placement on the body or in the environment (Column 6), the machine learning/deep learning/artificial intelligence models utilized (Column 7), the number of subjects involved in data collection (Column 8), the performed activities (Column 9), the total number of activities (Column 10), and the type of environment considered (Column 11).

Instead, Tables \ref{tab:S-DD-1}, \ref{tab:S-ED-1}, \ref{tab:S-H-1}, \ref{tab:H-DD-1}, and \ref{tab:H-ED-1} provide the annotation techniques used by the individual publications, and summarizes the individual advantages (Column 3) and disadvantages (Column 4) of every approach.

\add{Furthermore, in order to enhance the readability of Tables 8 to 17, an overview of the glossary used to identify the various types of activities covered in the methodologies of the reviewed papers is presented in Table \ref{tab:glossary}.}

\begin{table}[!ht]
\centering
\caption{Glossary of used abbreviations to categorize the different human activities/status types.}\label{tab:glossary}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|l|p{9cm}}
\hline
\textbf{Acronym} & \textbf{Extended} & \textbf{Definition}\\
\hline\hline
\textbf{BHA} & Basic Human Activities & The class of activities comprising \emph{walking}, \emph{running}, and \emph{sleeping} can be broadly defined as ``basic human activities''. These activities are fundamental to human life and are integral parts of our daily routines.\\
\hline
\textbf{OBI} & Object-based Interactions & The class of activities comprising interactions with objects such as \emph{smartphones} or \emph{fridges} can be referred to as ``object-based interactions''. These activities involve engaging with specific objects to perform various tasks or actions.\\
\hline
\textbf{ADL} & Activities of Daily Living &  ADLs are a set of essential everyday activities that individuals typically perform as part of their daily routines to maintain their personal well-being and independence. These can be: personal hygiene, eating, or cooking.\\
% These activities are fundamental for basic self-care and are often used as a measure to assess an individual's functional abilities and overall level of independence. \\
\hline
\textbf{PA} & Protocol Activities & Human activities within an experimental protocol refer to activities that individuals were asked to carry out solely for the study. They can vary depending on the specific nature of the experiment and the research objectives.\\
\hline
\textbf{R} & Risky & Risky activities refer to actions or behaviors that involve an increased potential for accidents, injuries, or negative outcomes. One example of a risky activity is falling.\\
\hline\hline
\end{tabular}}
\end{table}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=.5\textwidth,page={7}]{img/figures.pdf}
%     \caption{Automatic data annotation taxonomy in HAR (2).}
%     \label{fig:}
% \end{figure}



\subsection{Semi-Automated Annotation}\label{sec:4.1}
Within this section, the 25 papers on semi-automated data annotation techniques for HAR are categorized into the three subcategories mentioned earlier, and their proposed methods and key features are described in detail.

\subsubsection{Data Centric-Based Annotation}\label{sec:4.1.1}
These studies propose semi-automated data-centric methodologies for HAR automated data annotation, leveraging various techniques such as active learning, automated labeling algorithms, augmented and transfer learning frameworks, and self-supervised learning. These methodologies aim to reduce the manual effort and cost involved in annotating large volumes of data, while improving the accuracy and performance of activity recognition models. Combining human expertise with automated processes provides efficient and effective solutions for labeling and analyzing human activities in diverse contexts and settings.
Tables \ref{tab:S-DD} and \ref{tab:S-DD-1} offer a comprehensive summary of the 15 identified works falling in such category.
% % \begin{landscape}
% \begin{table}[!th]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c||c
% p{1.1cm}
% p{2cm}
% p{2cm}
% p{1.15cm}
% p{2cm}
% p{3cm}
% p{2cm}
% p{5cm}
% p{1cm}
% p{1.1cm}||
% p{4cm}
% p{4cm}
% p{4cm}}
% \hline
% \makecell{Ref.\\ (Year)} & \makecell{Dataset\\Owner} & \# of\newline Datasets & Devices & Sensors & \# of\newline Sensors & Position & Model & \# of Subjects [M/F] & Activities & \# of Activities & \makecell{In-Out\\ Door}& Annotation & Advantages & Limitations \\ \hline \hline
% \cite{saeedi2017co}\\ (2017)
% &No
% &1
% &IMU
% &Accelerometer, Gyroscope
% &7
% &chest, shin, forearm, thigh, upper-arm, head, and waist
% &k-NN\newline DT\newline RF
% &15[8/7]
% &Walking, Running, Sitting, Standing, Stair down, Stair up, Jumping, and Lying
% &8
% &Indoor
% &Transfer/Active-Learning
% &The accuracy of activity recognition reaches over 85\% by labeling only 15\% of unlabeled data
% &Requires 15\% of labeled data\\ \hline

% \cite{martindale2018smart}\\ (2018)
% &Yes
% &1
% &IMU, VIDEO, Pressure Insoles
% &Accelerometer, Gyroscope, Pressure
% &7
% &taurus, wrists, shoe side, under-feets
% &Threshold
% &20[15/5]
% &writing, straight walking, jogging and running, zigzagging between three tables, standing, sitting, jumping, jumping jacks, skipping, stepping, hopping, side steps, jumping over a line, zigzagging between cones, high kick running
% &13
% &Indoor\newline Outdoor
% & Four methods: 1) EdgeDet1: Detection of rising and falling edges of the individual pressure sensors.\newline
% 2) EdgeDet2: Detection of rising and falling edges of all 5 pressure sensors’ profiles.\newline
% 3) Threshold: De-drift using envelope subtraction, followed by detection of threshold crossings.\newline
% 4) Moticon: Moticon algorithm based on 100 Hz data
% & Uses the recognition of walking cycles phase to recognize the activities. \newline
% & Feedback is required to validate the inferred label and 17\% manual labeling or correction required.\\ \hline

% \cite{gan2018automatic}\\ (2018)
% &Yes
% &1
% &Smartphone, Smartwatch
% &Accelerometer
% &2
% &wrist
% &SVM\newline RF\newline K-NN\newline NN
% &1
% &fall
% &1
% &Indoor
% & Threshold-based and Clustering
% &Produced a fall detection accuracy of up to 97\%, and automatic labeling of peak-trough magnitudes  resulted in a step counting accuracy of at least 96\%
% &Requires feedback from the observer to identify a few fall contexts \\ \hline

% \cite{bota2019semi}\\ (2019)
% &No
% &2
% &IMU
% &Accelerometer, Gyroscope
% &1-4
% &waist - right/left hand, right ankle, and right side of the waist
% &Semi-Supervised\newline Active Learning\newline (SSAL)
% &30 - 12
% &laying, sitting, standing, walking, upstairs and downstairs - laying, sitting, standing, running, walking, upstairs and downstairs
% &6 - 7
% &Indoor
% &Semi-Supervised Active Learning
% &Reduces the required annotated data by more than 89\%
% &Requires labeled data\\ \hline

% \cite{martindale2019hidden}\\ (2019)
% &Yes
% &1
% &IMU
% &Accelerometer, Gyroscope
% &5
% &taurus, wrists, shoe side, under-feets
% &
% &80[52/28]
% &writing, straight walking, jogging and running, zigzagging between three tables, standing, sitting, jumping, jumping jacks, skipping, stepping, hopping, side steps, jumping over a line, zigzagging between cones, high kick running
% &12
% &Indoor
% &Annotate data from 20 subjects, train an hHMM, use the model to annotate data from the next 10 subjects, correct the annotations, and retrain the hHMM with the 30 subjects, and ahead with the next 10 subjects. 
% &Reduces the annotation time to only 15\%.
% &Requires 15\% of labeled data. \\ \hline


% \cite{ponnada2019designing}\\ (2019)
% &Yes
% &1
% &Actigraph
% &Accelerometer
% &1
% &wrist
% &Mobots and \newline Signaligner \newline games
% &50
% &walking, running, sitting, resting, working on PC, sleep
% &6
% &Indoor
% &Annotate activities in real-time using a custom, tablet-based application 
% & Reduces annotation time 
% & Pre-labeled data are used as baseline \\ \hline

% \cite{faridee2019augtoact}\\ (2019)
% &Ni
% &2
% &Smartphone, Smartwatch
% &Accelerometer
% &8-4
% &chest, head, shin, thigh, upper arm waist - NA
% &Augmentaiton \newline model \newline (AugToAct) 
% &15 / NA
% &biking, sitting, standing, walking, stair-sup, stairs-down - dance
% &6 - 10
% &Indoor\newline Outdoor
% &Semi-Supervised /Transfer Learning module + Augmentation model
% &Requires a low amount of labeled data
% &Requires labeled data\\ \hline

% \cite{hossain2019active}\\ (2019)
% &Yes
% &1
% &Smartphone
% &Accelerometer
% &1
% &front pant pocket
% &Deep-Active \newline Learning and \newline Actor-Critic \newline Network
% &20[14/6]
% &walking, eating, running, working, sitting, standing
% &6
% &Indoor\newline Outdoor
% &Actor-Critic Network That annotates data based on the part of the data manually annotated starting from videos and annotated by the users from the mobile app. 
% &Requires less than 30\% of labeled data to maintain the same results obtained by the 100\% labeled data
% & Requires interaction with the users and requires starting labeled data. \\ \hline

% \cite{sawano2020annotation}\\ (2020)
% &Yes
% &1
% &Smartphone
% &Accelerometer
% &1
% &hand, on a table, pocket, walking, using the smartphone, standing 
% &Semi-Supervised Learning
% &5
% &smartphone unused in a hand, using the smartphone and placing  it on a table, leaving the smartphone unused on a table, holding the smartphone and using it, standing with the smartphone in a pocket, walking while holding the smartphone unused in a hand, walking while using the smartphone, smartphone in chest pocket, leaving the smartphone unused on a bed, standing with the smartphone in a bag  
% &10
% &Indoor
% &Smartphone app that collects data and annotates the users response to notifications
% &Reduced annotation time
% &User intervention and labeled data are required\\ \hline 

% \cite{kwon2020imutube}\\ (2020)
% &No
% &2 IMU, 9 Video
% &Virtual IMU
% &Accelerometer, Gyroscope
% &11-3
% &left and right feet, left shin and thigh, hip, back, left and right arms, left and right forearms - NA
% &DeepConv \newline LSTM
% &9 - 14
% &stand, walk, sit, lie, ascending stairs, descending stairs, rope jumping, lying, running, sitting, standing, walking
% &11 - 8
% &Indoor\newline Outdoor
% &utilize existing, large-scale video repositories from which we generate virtual IMU data that are then used for training the HAR system 
% &Generates IMU data from video
% &Requires a training stes comprising vido and IMU streams\\ \hline

% \cite{avsar2021benchmarking}\\ (2021)
% &No
% &1
% &Video
% &\textit{na}
% &\textit{na}
% &\textit{na}
% &Temporal \newline Convolutional\newline Neural-Network
% &14
% &Standing, Walking, Cart, Handling (upward), Handling (centered), Handling (downward), Synchronization, and None.
% &8
% &Indoor
% &Semiautomated annotation consists of a combination of predictions from the CNN-IMU and a human revision
% &Reduced annotation time
% &Requires human revision\\ \hline

% \cite{korpela2021reducing}\\ (2021)
% &No
% &4
% &Video
% &\textit{na}
% &\textit{na}
% &\textit{na}
% &Simple Linear\newline Iterative \newline Clustering (SLIC) \newline and Image \newline Segmentation\newline  Algorithm
% &\textit{na}
% &standing sitting, laying walking, walking upstairs, walking downstairs, stand to sit, sit to stand, sit to lie, lie to sit, stand to lie, lie to stand 
% - open fridge, close fridge, open dishwasher, close dishwasher, open drawer 1, close drawer 1, open drawer 2, close drawer 2, open drawer 3, close drawer 3, open door 1, close door 1, open door 2, close door 2, toggle switch, clean table, drink from cup none 
% - stand, walk, lie, sit, none
% - screw, wrench, stir, transfer, paint
% &12 - 18 - 5 - 5
% &Indoor
% &Semi-automatic Labeling Process
% &Reduced annotation time
% &Requires human revision\\ \hline

% \cite{tang2021selfhar}\\ (2021)
% &No
% &8
% &IMU
% &Accelerometer, Gyroscope
% &2 - 1 - 1 - 1 - 1 - 1 - 1 - 1
% &waist, arm - front pocket - front pocket - wrist - front pocket - waist - front pocket - wrist
% &Self-training \newline and \newline Self-Supervised \newline Learning \newline (SelfHAR)
% &9 - 24 - 66 - 28 - 30 - 30 - 29 - 2096
% &biking, sitting, standing, walking, walking upstairs and walking downstairs - 12 ADLs + 4 falls - sitting, standing, walking, walking upstairs, walking downstairs, lying, cycling, home activities, office activities, personal care and shopping - 9 ADLs + 8 Falls - walking, walking upstairs, walking downstairs, sitting, standing and laying down - walking, jogging, sitting, standing, walking upstairs and walking downstairs  - NA
% &6 - 6 - 11 - 11 - 9 - 6 - 6 - NA
% &Indoor\newline Outdoor
% &The pipeline adopts a teacher-student setup, where a teacher model is first trained and distills the knowledge of labeled data by labeling a large unlabeled dataset
% &Reduced annotation time and tested on 9 different HAR datasets
% &Requires human revision\\ \hline 

% \cite{yhdego2022fall}\\ (2022)
% &Yes
% &1
% &VR headset
% &Accelerometer, Gyroscope
% &1
% &shank
% &Deep Residual \newline Network (ResNet)
% &16[14/2]
% &falls
% &1
% &Indoor
% &Use VR falls to capture real falls
% &Realistic falls
% &Labeled Data are generated \\ \hline

% \cite{mohamed2022har}\\ (2022)
% &No
% &2
% &Smartwatch
% &IMU, HR
% &3-4
% & NA - NA
% &HAR-graphs is\newline deep Graph CNNs \newline (GCNNs)
% &60 - 9
% &sitting, sleeping, strolling, cooking - NA
% &51 - 12 
% &Indoor
% &HAR-GCNN is a graph comprised of partially labeled sensor measurements that are chronologically ordered activities 
% &Improving classification accuracy by about 25\% and up to 68\% on different datasets
% &Requires user intervention
% \\
% \hline \hline
% \end{tabular}}
% \caption{Semi-automated Data-Driven Approaches in Automatic Data Annotation for HAR methodologies.}\label{tab:S-DD}
% \end{table}
% %\end{landscape}

\begin{table}[!th]
\centering
\caption{Semi-automated Data-Driven approaches.}\label{tab:S-DD}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||cccccccccc}
\hline
\makecell{\textbf{Ref.}\\ \textbf{(Year)}} & \makecell{\textbf{Dataset}\\\textbf{Owner (\#)}} & \textbf{Devices} & \textbf{Sensors} & \makecell{\textbf{\# of}\\ \textbf{Sensors}} & \textbf{Position} & \textbf{Model} & \makecell{\textbf{\# of} \\\textbf{Subjects [M/F]}} & \textbf{Activities} & \makecell{\textbf{\# of} \\\textbf{Activities}} & \makecell{\textbf{In/Out}\\ \textbf{Door}}\\ \hline \hline
\makecell{\cite{saeedi2017co}\\ (2017)}
&no (1)
&IMU
&\makecell{accelerometer,\\ gyroscope}
&7
&\makecell{chest, shin, forearm,\\ thigh, upper-arm, head,\\ and waist}
&\makecell{k-NN\\ DT\\ RF}
&15[8/7]
% &\makecell{walking, running, sitting,\\ standing, stair down, stair up,\\ jumping, and lying}
&\makecell{BHA}

&8
&indoor\\ \hline

\makecell{\cite{martindale2018smart}\\ (2018)}
&yes (1)
&\makecell{IMU, video,\\ pressure\\ insoles}
&\makecell{accelerometer,\\ gyroscope,\\ Pressure}
&7
&\makecell{taurus, wrists, shoe\\ side, under-feet}
&Threshold
&20[15/5]
% &\makecell{writing, straight walking, jogging\\ and running, zigzagging between\\ three tables, standing,\\ sitting, jumping, jumping jacks,\\ skipping, stepping, hopping,\\ side steps, jumping over\\ a line, zigzagging between\\ cones, high kick running}
&\makecell{BHA, PA}
&13
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{gan2018automatic}\\ (2018)}
&yes (1)
&\makecell{smartphone,\\ smartwatch}
&accelerometer
&2
&wrist
&\makecell{SVM, RF,\\ K-NN, NN}
&1
% &fall
& R
&1
&indoor\\ \hline

\makecell{\cite{bota2019semi}\\ (2019)}
&no (2)
&IMU
&\makecell{accelerometer,\\ gyroscope}
&1-4
&\makecell{waist - right/left hand,\\ right ankle, and right\\ side of the waist}
&\makecell{Semi-Supervised\\ Active Learning\\ (SSAL)}
&30 - 12
% &\makecell{laying, sitting, standing,\\ walking, upstairs and downstairs\\ - laying, sitting, standing, running,\\ walking, upstairs and downstairs}
&\makecell{BHA}
&6 - 7
&indoor\\ \hline

\makecell{\cite{martindale2019hidden}\\ (2019)}
&yes (1)
&IMU
&\makecell{accelerometer,\\ gyroscope}
&5
&\makecell{taurus, wrists, shoe\\ side, under-feet}
& HMM
&80[52/28]
% &\makecell{writing, straight walking, jogging\\ and running, zigzagging between\\ three tables, standing, sitting,\\ jumping, jumping jacks, skipping,\\ stepping, hopping, side steps,\\ jumping over a line, zigzagging\\ between cones, high kick running}
&\makecell{BHA, PA, OBI}
&12
&indoor\\ \hline


\makecell{\cite{ponnada2019designing}\\ (2019)}
&yes (1)
&actigraph
&accelerometer
&1
&wrist
&\makecell{Mobots and\\ Signaligner games}
&50
% &\makecell{walking, running, sitting,\\ resting, working on PC, sleep}
&\makecell{BHA, OBI}
&6
&indoor\\ \hline

\makecell{\cite{faridee2019augtoact}\\ (2019)}
&no (2)
&\makecell{smartphone,\\ smartwatch}
&accelerometer
&8-4
&\makecell{chest, head, shin,\\ thigh, upper arm waist - NA}
&\makecell{Augmentatiton model\\ (AugToAct)} 
&15 / NA
% &\makecell{biking, sitting, standing,\\ walking, stair-sup,\\ stairs-down - dance}
&\makecell{BHA}
&6 - 10
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{hossain2019active}\\ (2019)}
&yes (1)
&smartphone
&accelerometer
&1
&front pant pocket
&\makecell{Deep-Active Learning\\ and Actor-Critic Network}
&20[14/6]
% &\makecell{walking, eating, running,\\ working, sitting, standing}
&\makecell{BHA}
&6
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{sawano2020annotation}\\ (2020)}
&yes (1)
&smartphone
&accelerometer
&1
&\makecell{hand, on a table, pocket,\\ walking, standing }
&\makecell{Semi\\ Supervised\\ Learning}
&5
% &\makecell{smartphone unused in a hand,\\ using the smartphone and placing\\ it on a table, leaving\\ the smartphone unused on a table,\\ holding the smartphone and\\ using it, standing with the smartphone\\ in a pocket, walking while\\ holding the smartphone unused\\ in a hand, walking while\\ using the smartphone, smartphone\\ in chest pocket, leaving the\\ smartphone unused on a bed,\\ standing with the smartphone\\ in a bag}
&\makecell{OBI}
&10
&indoor\\ \hline 

\makecell{\cite{kwon2020imutube}\\ (2020)}
&no (11)
&\makecell{virtual\\ IMU}
&\makecell{accelerometer,\\ gyroscope}
&11-3
&\makecell{left and right\\ feet, left shin and\\ thigh, hip, back, left\\ and right arms, left \\and right forearms - NA}
&\makecell{DeepConv\\ LSTM}
&9 - 14
% &\makecell{stand, walk, sit, lie,\\ ascending stairs, descending stairs,\\ rope jumping, lying, running,\\ sitting, standing, walking}
&\makecell{BHA}
&11 - 8
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{avsar2021benchmarking}\\ (2021)}
&no (1)
&video
&\textit{na}
&\textit{na}
&\textit{na}
&\makecell{Temporal\\ Convolutional\\ Neural-Network}
&14
% &\makecell{standing, walking, cart,\\ handling (upward), handling\\ (centered), handling (downward),\\ synchronization, and none.}
&\makecell{BHA, PA}
&8
&indoor\\ \hline

\makecell{\cite{korpela2021reducing}\\ (2021)}
&no (4)
&video
&\textit{na}
&\textit{na}
&\textit{na}
&\makecell{Simple Linear\\ Iterative Clustering and\\ Image Segmentation Algorithm}
&\textit{na}
% &\makecell{standing sitting, laying walking,\\ walking upstairs, walking downstairs,\\ stand to sit, sit to stand,\\ sit to lie, lie to sit,\\ stand to lie, lie to stand\\ 
% - open fridge, close fridge,\\ open dishwasher, close dishwasher,\\ open drawer 1, close drawer 1,\\ open drawer 2, close drawer 2,\\ open drawer 3, close drawer 3,\\ open door 1, close door 1,\\ open door 2, close door 2,\\ toggle switch, clean table,\\ drink from cup none 
% - stand,\\ walk, lie, sit, none
% - screw,\\ wrench, stir, transfer, paint}
&\makecell{BHA, ADL, OBI}
&12 - 18 - 5 - 5
&indoor\\ \hline

\makecell{\cite{tang2021selfhar}\\ (2021)}
&no (8)
&IMU
&\makecell{accelerometer,\\ gyroscope}
&\makecell{2 - 1 - 1 \\- 1 - 1 - 1\\ - 1 - 1}
&\makecell{waist, arm - front pocket\\ - front pocket - wrist\\ - front pocket - waist\\ - front pocket - wrist}
&\makecell{Self-training and\\ Self-Supervised \\Learning (SelfHAR)}
&\makecell{9 - 24 - 66\\ - 28 - 30 - 30\\ - 29 - 2096}
% &\makecell{biking, sitting, standing, walking,\\ walking upstairs and walking downstairs\\ - 12 ADLs + 4 falls\\ - sitting, standing, walking, walking\\ upstairs, walking downstairs, lying,\\ cycling, home activities, office\\ activities, personal care and shopping\\ - 9 ADLs + 8 Falls - walking,\\ walking upstairs, walking downstairs,\\ sitting, standing and laying down \\- walking, jogging, sitting, standing,\\ walking upstairs and walking downstairs - NA}
&\makecell{BHA, ADL, R}
&\makecell{6 - 6 - 11\\ - 11 - 9 - 6\\ - 6 - NA}
&\makecell{indoor\\ outdoor}\\ \hline 

\makecell{\cite{yhdego2022fall}\\ (2022)}
&yes (1)
&VR headset
&\makecell{accelerometer,\\ gyroscope}
&1
&shank
&\makecell{Deep Residual\\ Network (ResNet)}
&16[14/2]
% &falls
& R
&1
&indoor\\ \hline

\makecell{\cite{mohamed2022har}\\ (2022)}
&no (2)
&smartwatch
&IMU, HR
&3-4
& NA - NA
&\makecell{Graph CNNs \\(GCNNs)}
&60 - 9
% &\makecell{sitting, sleeping,\\ strolling, cooking - NA}
&\makecell{BHA}
&51 - 12 
&indoor\\ \hline \hline
\multicolumn{11}{c}{"-" in Columns \# of Sensors, Position, \# of Subjects [M/F], Activities, and \# of Activities separates the info of the different datasets.}
\end{tabular}}
\end{table}

% \begin{landscape}
\begin{table}[!th]
\centering
\caption{Annotation methods, Advantages, and Limitations of Semi-automated Data-Driven approaches.}\label{tab:S-DD-1}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||p{8cm}p{6cm}p{6cm}}
\hline
\textbf{Ref. (Year)} & \textbf{Annotation} & \textbf{Advantages} & \textbf{Limitations} \\ \hline \hline
\makecell{\cite{saeedi2017co}\\ (2017)}
& Transfer/Active Learning
& The accuracy of activity recognition reaches over 85\% by labeling only 15\% of unlabeled data.
& Requires 15\% of labeled data.\\ \hline

\makecell{\cite{martindale2018smart}\\ (2018)}
& Four methods: 1) EdgeDet1: Detection of rising and falling edges of individual pressure sensors.\newline
2) EdgeDet2: Detection of rising and falling edges of all 5 pressure sensors’ profiles.\newline
3) Threshold: De-drift using envelope subtraction, followed by detection of threshold crossings.\newline
4) Moticon: Moticon algorithm based on 100 Hz data.
& Uses walking cycle phase recognition to identify activities.
& Requires feedback for label validation, and 17\% manual labeling or correction is needed.\\ \hline


\makecell{\cite{gan2018automatic}\\ (2018)}
& Threshold-based and Clustering
& Achieves up to 97\% fall detection accuracy and at least 96\% step counting accuracy with automatic labeling of peak-trough magnitudes.
& Requires observer feedback to identify some fall contexts.\\ \hline

\makecell{\cite{bota2019semi}\\ (2019)}
&Semi-Supervised Active Learning
&Reduces the required annotated data by more than 89\%.
&Requires labeled data.\\ \hline

\makecell{\cite{martindale2019hidden}\\ (2019)}
& Annotates data from 20 subjects, trains an hHMM, uses the model to annotate data from the next 10 subjects, corrects the annotations, and retrain the hHMM with the 30 subjects, and so on.
& Reduces annotation time to only 15\%.
& Requires 15\% of labeled data. \\ \hline

\makecell{\cite{ponnada2019designing}\\ (2019)}
& Real-time activity annotation with a custom tablet app.
& Decreases annotation time.
& Baseline requires pre-labeled data.\\ \hline

\makecell{\cite{faridee2019augtoact}\\ (2019)}
&Semi-Supervised /Transfer Learning module + Augmentation model
&Requires a low amount of labeled data
&Requires labeled data\\ \hline

\makecell{\cite{hossain2019active}\\ (2019)}
& Actor-critic network that annotates data based on the part manually annotated starting from videos and annotated by the users from the mobile app. 
& Maintains the same results obtained with 100\% labeled data using less than 30\% labeled data.
& Requires user intervention and labeled data.\\ \hline

\makecell{\cite{sawano2020annotation}\\ (2020)}
& Smartphone app that collects data and annotates users' response to notifications.
& Reduces the annotation time.
& Requires user feedback and labeled data.\\ \hline

\makecell{\cite{kwon2020imutube}\\ (2020)}
& Utilizes existing large-scale video repositories to generate virtual IMU data for training the HAR system.
& Generates IMU data from video.
& Requires a training set comprising of video and IMU data.\\ \hline

\makecell{\cite{avsar2021benchmarking}\\ (2021)}
& Semiautomated annotation combining predictions from CNN-IMU with human revision.
& Reduces annotation time.
& Requires human revision.\\ \hline

\makecell{\cite{korpela2021reducing}\\ (2021)}
& Semi-automatic Labeling Process
& Reduces annotation time.
& Requires human revision.\\ \hline

\makecell{\cite{tang2021selfhar}\\ (2021)}
& Adopts a teacher-student setup where a teacher model distills knowledge from labeled data by annotating a large unlabeled dataset.
& Reduces annotation time and was tested on 9 different HAR datasets.
& Requires human revision.\\ \hline

\makecell{\cite{yhdego2022fall}\\ (2022)}
& Uses VR falls to capture real falls.
& Provides realistic falls.
& Uses synthetically generated labels.\\ \hline

\makecell{\cite{mohamed2022har}\\ (2022)}
& HAR-GCNN is a graph comprised of partially labeled sensor measurements that represent chronologically ordered activities.
& Improves the classification accuracy by about 25\% and up to 68\% on different datasets.
& Requires user intervention.\\\hline \hline
\end{tabular}}
\end{table}

In~\cite{saeedi2017co}, Saeedi et al. proposed a new architecture for managing a multi-expert mobile health (M-health) system using active learning. This architecture addressed several challenges and scenarios associated with reconfiguring mobile sensor devices for health monitoring. One such challenge was the cost of data labeling in the learning process, which could be expensive due to interference in the user's life, feedback from healthcare experts, or equipment cost. Another challenge was the unknown suitable expert for each data instance, and the third challenge was the uncertainty of labels due to limited expert knowledge. To overcome these challenges, the proposed architecture found a cost-optimal and most-confident expert for each query while considering collaboration among experts to minimize cost and gain more accurate data labeling. The authors also developed new algorithms for expert selection and system initialization, employing available clustering algorithms and ensemble classification methods. The efficacy of the architecture and algorithms were demonstrated using activity monitoring as a case study, achieving an accuracy of activity recognition as high as 85\% by labeling only 15\% of unlabeled data while reducing annotation cost through cost-optimal expert selection and expert collaboration. Future work includes enhancing the architecture to handle multi-modality sensory systems and using the system in a real pilot study of an intervention system. Additionally, the authors plan to integrate transfer learning and active learning approaches to reduce the number of queries further and increase the learner's accuracy.


In \cite{martindale2018smart}, Martindale et al. proposed a pipeline for data collection that allows for semi-automated labeling and efficient collection of daily activity data labeled on a walking cycle level recognition. Although the setup was still somewhat controlled, the same principles could be applied to more natural or specific applications. They proposed an on the edge detection method to detect on-the-ground, off-the-ground stride phases with only 17\% manual labeling or correction required. %These two contributions were combined into a smart annotation tool, which is being used as the basis of an ongoing large dataset collection. 
This tool reduced labeling time by 83\% compared to complete manual labeling without assistance. The authors plan to use this methodology to label large volumes of IMU data and produce a benchmark dataset useful for validating gait events occurring within natural settings. They believe that the dataset and annotation tool will also be useful for validating IMU-based home monitoring algorithms or those designed for "in the wild" use. Additionally, they plan to use it to train and validate semi-supervised or even unsupervised algorithms for segmenting and classifying cyclic human motion using wearable sensors.


Gan et al., in \cite{gan2018automatic}, put forward an approach that utilized automatic labeling algorithms to personalize wearable monitoring models. They devised two automated labeling algorithms for this purpose: one for personalized fall detection online model training using K-means clustering and another for personalized localization online model training that employed a descendingly ordered set of peak-trough magnitudes. Based on their experiments, the authors reported that the automatic labeling approach using the maximum sum of cluster means resulted in a fall detection accuracy of up to 97\%. In contrast, the automatic labeling of peak-trough magnitudes led to a step counting accuracy of at least 96\%. Although their approach mitigated the issue, it did not completely address it.

%--pk
Bota et al., in \cite{bota2019semi}, proposed a semi-automatic data annotation approach to address the challenges posed by the significant volume of data recorded by unobtrusive and pervasive sensors such as smartphones and wearables. The proposed approach consists of two steps: (1) selecting the most relevant samples to be labeled by an expert using a QS criterion, and (2) propagating the annotated sample's label over similar samples on the entire dataset using an automatic method. 
The study's main contribution was the application of Semi-Supervised Active Learning (SSAL) to two HAR datasets, using a comprehensive study of state-of-the-art Query Strategies (QSs) and Stopping Criteria (SCs), and a comparison to Active Learning (AL). The methods were evaluated over several automatic annotation strategies based on different distance functions to build an optimal SSAL system for human movement. Margin Sampling achieved the best results in the study performed with AL, while Self-Training-SSAL (ST-SSAL) using the Over-CC SC achieved a similar classification performance to AL, but was able to annotate a higher volume of data with similar annotation effort. 
This paper extended the work conducted by \cite{stikic2009activity} on HAR by applying ST on the labels previously selected by AL. The authors identified future research directions, including developing a multi-oracle system with non-expert users, integrating the samples' estimation annotation cost into the QS, and development of an annotation interface that relies on ST-SSAL to facilitate data annotation. This annotation interface can be used to support current methods based on video recordings, reducing the annotation effort required by the user.


In \cite{martindale2019hidden}, Martindale et al. proposed a smart annotation pipeline to overcome the current lack of realistic and labeled datasets for medical applications of cyclic activity monitoring, such as step-counting and gait analysis. The pipeline reduces the percentage of labels that require manual adjustment to only 14\%, making it possible to produce a public dataset of over 150,000 labeled cycles from 80 participants. The dataset includes 12 activities, 10 of which are cyclic, and features diverse ranges of bouts, transitions, and non-straight walking. For datasets such as home monitoring, where mostly walking data is expected, the labeling effort for new datasets can be as low as 8\%. The authors believe that the smart annotation pipeline and dataset will be helpful for benchmarking semi- and unsupervised learning algorithms as well as simultaneous segmentation and classification algorithms. Furthermore, the authors proposed an iterative training technique for a hierarchical Hidden Markov Model (hHMM) in this paper. The hHMM hierarchy now includes cycle phases for each of the 10 cyclic activities, and this method enabled the dataset made public in \cite{martindale2018smart} to be expanded fourfold with a final miss rate of 0.6\% and false discovery rate of 7.6\%. The complete pipeline achieved an F1-score of 89.5\% with an expected accuracy for new data of F1-score 93.0\%. This pipeline can expand existing datasets with significantly less labeling effort, and the current dataset and pipeline can be used as a benchmarking tool for further smart annotation pipelines focusing on cycle analysis in human motion.

In \cite{ponnada2019designing}, Ponnada et al., proposed two Human Computation Games (HCG) design prototypes, Mobots and Signaligner, with the aim of motivating players to label raw accelerometer data. The feasibility of the games was assessed using MTurk players, and it was found that Signaligner players showed higher labeling accuracy and inter-player agreement compared to Mobots players. This was attributed to the fact that in Signaligner, players were provided with more signal context and visual patterns to match with an on-screen reference. In contrast, Mobots players were required to rely on their memory of signals and activity categories to label short fragments of data. Both games had low tolerance for errors at transitions, and the authors suggested allowing more tolerance for transitions in the initial levels to improve the gaming experience. Moreover, the authors proposed that game players could help to verify or fix computer-generated labels and identified three ways in which an activity recognition algorithm and labels by casual game players could be combined to produce well-labeled training data. Finally, the authors highlighted the potential of crowd-based labeling systems to label data where the algorithms are uncertain, but this strategy requires that the algorithms be capable of outputting inferred labels and likelihoods.

Faridee et al.\cite{faridee2019augtoact}  introduced the AugToAct framework, a flexible and innovative semi-supervised transfer learning framework with augmented capabilities. The framework can be applied to different classification and domain adaptation tasks, showcasing its suitability for complex HAR. However, the data augmentation methodology described in the study lacks guidance, and the optimal parameter values were determined through empirical experimentation. The authors aim to automate the process of identifying optimal augmentation parameters in future research. Additionally, they plan to evaluate the model's generalizability on a broader range of datasets encompassing diverse human activities. Furthermore, they intend to involve users with varying training and dexterity levels to explore the scalability challenges of complex HAR. Notably, the current experiment does not address unseen labels in the target domain, a limitation the authors plan to overcome in their future work. 


In \cite{hossain2019active}, Hossain et al., proposed a deep model for activity recognition that incorporates active learning in hyperparameter tuning, as opposed to previous works that only focused on identifying the most informative instance through active learning. To achieve this, the authors suggested optimizing network parameters using a joint loss function that combined the cross-entropy loss of the deep model and the entropy function of the active learning pipeline. To validate their approach, they used their mobile application to collect data in real-world settings, and the results showed that the joint loss function helped the deep model to generalize better with lower weight values, even in the presence of outliers. 
The authors also introduced a novel annotator selection model based on the contextual similarity between annotators and users, outperforming other algorithms by converging faster to optimal accuracy. In their future work, the authors intend to investigate constraints like query budget and annotator availability in their annotator selection model, as they were not considered in the current work.


Sawano et al. \cite{sawano2020annotation} proposed a method for estimating user and device situations based on user responses to notifications generated by a smartphone. The evaluation experiment showed that the proposed method had an average precision of 76.9\% and 96.3\% for user-independent and user-dependent experiments, respectively. Although the proposed method had high annotation precision, the recall was low, meaning that accurate annotation can only be given to a limited amount of data. However, since the method has an automatic annotation collection mechanism, it can collect a large amount of annotated data for many people over a long period of time, even if the recall is small.
% The paper also discussed limitations, such as the assumption of only a few situations, and the need for training data for new annotations. The proposed system needs to learn the data with the target clothes to annotate the data. However, if the proposed system has not learned the data with several users' clothes, the system will not give annotations to the data rather than giving incorrect annotation.
% In conclusion, the proposed method showed promising results, and future studies will investigate the method's effectiveness in various unexpected situations, evaluate the improvement in the performance of the classifier using the proposed method's annotated data, and verify the method in other user-independent situations. A scaled investigation with many users recruited through crowdsourcing for the long term is also planned.


In \cite{kwon2020imutube}, Kwon et al. proposed a solution to the lack of labeled data in HAR by introducing IMUTube. This automated processing pipeline generates virtual streams of IMU data from human activity videos. By integrating computer vision and signal processing techniques, the proposed framework overcomes the challenge of annotating the data, which is time-consuming and error-prone. The authors demonstrated the effectiveness of the virtually-generated IMU data in improving the performance of existing HAR models. While the initial results are promising, the authors suggest a collective approach by the computer vision, signal processing, and activity recognition communities to extend this work and build on the IMUTube pipeline. 


Avsar et al. \cite{avsar2021benchmarking} present a semi-automated annotation approach for generating high-quality data in the context of multi-channel time series HAR. Their method utilizes optical motion capturing and inertial measurements from on-body devices to combine temporal CNN predictions with manual revisions, resulting in fine-grained annotations.
The study demonstrates that this semi-automated approach significantly reduces the effort required for annotation while maintaining comparable quality to manual annotation.
Furthermore, the authors expand the existing HAR dataset for warehousing by capturing measurements from unseen target subjects and annotating human activities and binary semantic attributes for experimental purposes. They evaluate the semi-automated annotation procedures in terms of time consumption and annotation consistency, revealing a substantial reduction in effort by up to 62.8\%. Additionally, the experiments indicate that incorporating manually annotated recordings from target subjects enhances the quality of annotations.
% The study also highlights that maintaining annotation consistency for both activity classes and attributes can be achieved through the deployment of the semi-automated annotation approach. The authors propose exploring different segmentation approaches to address limitations related to determining the start and end points of activities. Additionally, they suggest leveraging confidence metrics from neural network predictions to aid in the manual revision process.


Korpela et al., in \cite{korpela2021reducing}, propose a novel technique to reduce label fragmentation in time-series data and improve the semi-automatic labeling process for HAR systems. They utilized an image segmentation algorithm called SLIC (Simple Linear Iterative Clustering) to perform temporal clustering of the classifier output. 
The time-series data was fed to the algorithm as a 1D image, with the class probabilities serving as the color channels. The proposed method was evaluated on 233 minutes of time-series data, and it achieved an average reduction of 56\% in annotation time compared to the baseline method that used raw classifier output. 

In \cite{tang2021selfhar}, Tang et al., proposed SelfHAR, a semi-supervised model that leverages unlabeled mobile sensing datasets to improve the performance of HAR models. SelfHAR uses a combination of teacher-student self-training and multi-task self-supervision to learn robust signal-level representations and augment small labeled datasets. SelfHAR was evaluated on various HAR datasets and found that it outperformed other supervised and semi-supervised approaches, achieving up to a 12\% increase in F1-score with the same number of model parameters at inference. Additionally, SelfHAR is data-efficient, achieving similar performance using up to 10 times less labeled data than supervised approaches. 
The authors suggest that their work improves the performance of deep learning models with limited labeled data and sheds light on how pre-training tasks can affect downstream performance. 


In their work on fall detection \cite{yhdego2022fall}, Yhdego et al. introduced a self-supervised learning approach that utilizes unlabeled data to pre-train Fully Connected Network (FCN) and Residual Neural Network (ResNet) models. These pre-trained models are then fine-tuned using labeled data. The method incorporates overlapping sliding windows for feature extraction and addresses the issue of imbalanced classes in the dataset through oversampling and a modified weighted focal loss function.
Experimental results demonstrated that the ResNet self-supervised deep learning method, combined with random oversampling, achieved an impressive average F1-score of 0.98 for accurately detecting falls compared to non-fall activities.
% Moving forward, the authors intend to enhance their approach by exploring the application of decorrelation of filter regularization to both networks. They also plan to conduct further investigations on the experimental data, model architecture, and hyperparameters to improve their methodology.


Mohamed et al., in \cite{mohamed2022har}, present HAR-GCCN (HAR-Graph Chronologically Correlation Network), a deep graph CNN model for HAR from mobile sensor data. 
They proposed leveraging the implicit chronology of human behavior to learn unknown labels and classify future activities by presenting a new training strategy that predicts missing activity labels by leveraging the known ones. 
HAR-GCCN outperformed previously used baseline methods, improving classification accuracy by up to 68\% on different datasets. In addition, they reported that HAR-GCNN has stable performance, independently of the number of chronologically ordered activities considered within the input graph.


% \newpage
\subsubsection{Environment-based}\label{sec:4.1.2}
The primary objective of these methodologies is to minimize the manual effort and expenses associated with annotating extensive datasets, while simultaneously enhancing the accuracy and performance of activity recognition models. 
By combining human expertise with automated processes, these approaches offer efficient and effective solutions for labeling and analyzing human activities across various contexts and environments.
Tables \ref{tab:S-ED} and \ref{tab:S-ED-1} offers a comprehensive summary of the articles in HAR's Semi-automated Environment-based category of automatic annotation systems.
% % \begin{landscape}
% \begin{table}[!th]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c||c
% p{1.1cm}
% p{2cm}
% p{2cm}
% p{1.15cm}
% p{2cm}
% p{3cm}
% p{2cm}
% p{5cm}
% p{1cm}
% p{1.1cm}||
% p{4cm}
% p{4cm}
% p{4cm}}
% \hline
% \makecell{Ref.\\ (Year)} & \makecell{Dataset\\Owner} & \# of\newline Datasets & Devices & Sensors & \# of\newline Sensors & Position & Model & \# of Subjects [M/F] & Activities & \# of Activities & \makecell{In-Out\\ Door}& Annotation & Advantages & Limitations \\ \hline \hline
% \cite{subramanya2012recognizing}\\ (2012)
% &Yes
% &1
% &Standalone
% &GPS, Accelerometer, 2 Microphones, Brightness, Temperature, Barometric 
% &7
% &Left shoulder
% &Graph \newline model 
% &6
% &stationary, walking, running, driving vehicle, going up/down stairs
% &6
% &Indoor\newline Outdoor
% &Utilizes a dynamic graphical model to jointly estimate both activity and spatial context over time
% &Uses environmental information to strengthen the annotation and context knowledge and achieves 95 \% accuracy in recognition of the studied activities
% &Requires labeled data\\ \hline

% \cite{woznowski2017talk}\\ (2017)
% &Yes
% &1
% &Smartphone
% &Mobile App, Voice, Location, NFC
% &1
% &\textit{na}
% &\textit{na}
% &\textit{na}
% & ADLs (Eating, working, drinking, etc)
% &\textit{na}
% &Indoor
% &A mobile app that reads the NFC tags attached to daily objects and places that (almost) automatically annotates the performed activity
% &Reduced effort for data annotation
% &Requires feedback from users\\ \hline

% \cite{tonkin2018talk}\\ (2017)
% &Yes
% &1
% &Smartphone
% &Mobile App, Voice, Location, NFC
% &1
% &\textit{na}
% &\textit{na}
% &10
% & ADLs (Eating, working, drinking, etc)
% &29
% &Indoor
% &A mobile app that reads the NFC tags attached to daily objects and places that (almost) automatically annotates the performed activity
% &Reduced effort for data annotation
% &Requires feedback from users\\ \hline

% \cite{solis2019human}\\ (2019)
% &Yes
% &1
% &Smartwatch
% &Bluetooth antenna
% &1
% &wrist
% &Graph-based \newline BLE-Location \newline Mapping
% &12
% &Eating
% &1
% &Indoor
% &Use Bluetooth device to recognize specific positions of the environment and ask the user (on their smartwatch) if they are performing a specific activity
% &Reduced effort for data annotation
% &Requires feedback from users\\
% \hline \hline
% \end{tabular}}
% \caption{Overview of Semi-automated environment-based methodologies.}\label{tab:S-ED}
% \end{table}
% % \end{landscape}

% \begin{landscape}
\begin{table}[!th]
\centering
\caption{Semi-automated environment-based approaches.}\label{tab:S-ED}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||cccccccccc}
\hline
\makecell{\textbf{Ref.}\\ \textbf{(Year)}} & \makecell{\textbf{Dataset}\\\textbf{Owner (\#)}} & \textbf{Devices} & \textbf{Sensors} & \makecell{\textbf{\# of}\\ \textbf{Sensors}} & \textbf{Position} & \textbf{Model} & \makecell{\textbf{\# of} \\\textbf{Subjects [M/F]}} & \textbf{Activities} & \makecell{\textbf{\# of} \\\textbf{Activities}} & \makecell{\textbf{In-Out}\\ \textbf{Door}}\\ \hline \hline
\makecell{\cite{subramanya2012recognizing}\\ (2012)}
&yes (1)
&standalone
&\makecell{GPS, accelerometer,\\ 2 microphones, brightness,\\ temperature, barometric} 
&7
&\makecell{left\\ shoulder}
&\makecell{Graph\\ model} 
&6
% &\makecell{stationary, walking,\\ running, driving vehicle,\\ going up/down stairs}
&\makecell{BHA, OBI}
&6
&Indoor\newline Outdoor
\\ \hline

\makecell{\cite{woznowski2017talk}\\ (2017)}
&yes (1)
&smartphone
&\makecell{mobile App, voice,\\ location, NFC}
&1
&\textit{na}
&\textit{na}
&\textit{na}
% &\makecell{ADLs (Eating, working,\\ drinking, etc)}
&\makecell{ADL}
&\textit{na}
&Indoor
\\ \hline

\makecell{\cite{tonkin2018talk}\\ (2017)}
&yes (1)
&smartphone
&\makecell{mobile app, voice,\\ location, NFC}
&1
&\textit{na}
&\textit{na}
&10
% &\makecell{ADLs (Eating, working,\\ drinking, etc)}
&\makecell{ADL}
&29
&Indoor
\\ \hline

\makecell{\cite{solis2019human}\\ (2019)}
&yes (1)
&smartwatch
&bluetooth antenna
&1
&wrist
&\makecell{Graph-based\\ BLE-Location Mapping}
&12
% &Eating
&\makecell{BHA}
&1
&Indoor
\\ \hline \hline
\multicolumn{11}{c}{"-" in Columns \# of Sensors, Position, \# of Subjects [M/F], Activities, and \# of Activities separates the info of the different datasets.}
\end{tabular}}
\end{table}
% \end{landscape}

% \begin{landscape}
\begin{table}[!th]
\centering
\caption{Annotation method, Advantage's, and Limitations of Semi-automated environment-based approaches.}\label{tab:S-ED-1}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||p{8cm}p{6cm}p{6cm}}
\hline
\textbf{Ref. (Year)} & \textbf{Annotation} & \textbf{Advantages} & \textbf{Limitations} \\ \hline \hline
\makecell{\cite{subramanya2012recognizing}\\ (2012)}
& Utilizes a dynamic graphical model to jointly estimate activity and spatial context over time.
& Achieves 95\% accuracy in recognizing activities by leveraging environmental information.
& Requires labeled data.\\ \hline

\makecell{\cite{woznowski2017talk}\\ (2017)}
& Mobile app that reads NFC tags on daily objects and places for almost automatic activity annotation.
& Reduces effort for data annotation.
& Requires user feedback.\\ \hline

\makecell{\cite{tonkin2018talk}\\ (2017)}
& Mobile app that reads NFC tags on daily objects and places for almost automatic activity annotation.
& Reduces effort for data annotation.
& Requires user feedback.\\ \hline

\makecell{\cite{solis2019human}\\ (2019)}
& Uses Bluetooth devices to recognize specific environmental positions and asks the user on their smartwatch if they are performing a specific activity.
& Reduces effort for data annotation.
& Requires user feedback.\\ \hline \hline
\end{tabular}}
\end{table}
% \end{landscape}


One of the first methodologies falling into such a category is from Szewcyzk et al. \cite{szewcyzk2009annotating}. In this work, the authors investigated four alternative mechanisms for annotating sensor data with corresponding activity labels to monitor the functional health of smart home residents. The first method utilizes the raw data from sensors along with a map of the apartment to identify the activities being performed. The location of the sensors and the time of day are used to infer the activities. For example, motion and water sensors triggered during a specific time could indicate meal preparation. 
In the second method, the residents provide time diaries reporting their activities every half hour. This approach is less invasive than others but relies on the residents' self-reports, which may not always be reliable.
The third and fourth methods involve using a visualization tool to analyze the sensor events. Method 3 uses the visualization tool, while Method 4 also includes resident feedback. A 3D environment simulator called CASASim displays sensor readings in real time. Researchers rely on the combined information from the simulator and resident time diaries to interpret and annotate the sensor events.

Subramanya et al., \cite{subramanya2012recognizing} proposed a new dynamic model for recognizing a person's activities and location using a small wearable sensor device. 
The model utilizes a dynamic graphical model to jointly estimate activity and spatial context over time based on asynchronous observations from GPS measurements and a sensor board. The joint inference is desirable as it improves the accuracy and consistency of the location and activity estimates. The model's parameters are trained on partially labeled data, and the authors applied virtual evidence to improve data annotation, providing high flexibility when labeling training data. 
The experiments show that the recognition accuracy of the proposed system is significantly higher than existing techniques that do not perform joint reasoning about a person's activities and spatial context. The proposed approach can correct GPS errors and achieve more consistent estimates of a person's location and environment context by taking information about the locations of buildings into account. In future work, the authors intend to develop a modeling language and graphical user interface that uses virtual evidence to model various types of user annotations. They also aim to improve the handling of GPS by better using maps and satellite images and investigating the use of Rao-Blackwellised particle filters better to represent a person's location in continuous space.


In the study conducted by Woznowski et al. \cite{woznowski2017talk} and  Tonkin et al. \cite{tonkin2018talk}, various approaches were explored to enable users to self-annotate their activities in near-real-time for the development of accurate HAR algorithms. 
The study proposed a mobile app with multiple logging approaches for self-annotation of activities. These approaches included model-based, voice-based, location-based, and NFC-based methods. Users interacted directly with the app, except for the NFC-based approach, which was fully automatic upon contact with NFC tags.

% In \cite{tonkin2018talk}, the authors suggested using self-annotation as a tool to capture accurate information in the real world through pervasive systems. The study explored the experiences of 12 people living in a smart home, who were provided with an app to annotate their activities and location. The results showed that self-annotation had both strengths and limitations. While it provided an opportunity for participants to reflect on themselves and their routines, it was not effective in capturing accurate start and finish times for activities, or location associated with activity information. The study recommended designing self-annotation tools that were meaningful and useful for all stakeholders in the process. It also suggested supporting post hoc self-annotation to increase data counts and enabling participants to identify some approximate time in the past to specify a post hoc annotation. The study further noted the challenge of acquiring accurate location information for activities correlated with a location and suggested exploring ways to better capture this type of information. Finally, the study observed that participants explored playful use of the app beyond a strict activity logging purpose.


In \cite{solis2019human}, Solis et al. propose a methodology to improve the recognition of eating moments using wearable computers in natural environments. They utilized location information from nearable sensors in IoT platforms to learn users' behavior patterns without prior knowledge. Annotations were requested only when automatic annotation failed. In a case study with 12 participants wearing smartwatches, audio recordings were used for labeling eating moments. The study showed a 2.4\% accuracy improvement with a limit of 20 requested annotations per day. %Incorporating environment information enhanced system accuracy, and the model continued to improve with more user annotations. Future work aims to predict nutrition intake and consider temporal shifts in labels. 
A dietary monitoring study validated the algorithm based on classifier uncertainty, allowing long-term data collection with minimal annotations.




\subsubsection{Hybrid}\label{sec:4.1.3}
The focus of hybrid methodologies is to further reduce manual effort and expenses associated with annotating extensive datasets while simultaneously enhancing the accuracy and performance of activity recognition models. 
% These approaches combine human expertise with automated processes to offer efficient and effective solutions for labeling and analyzing human activities across various contexts and environments. 
By leveraging this hybrid approach, the aim is to achieve more efficient data annotation and analysis, leading to improved HAR outcomes. Tables \ref{tab:S-H} and \ref{tab:S-H-1} provides an
overview of the methodologies falling into such category. 

% %\begin{landscape}
% \begin{table}[!th]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c||c
% p{1.1cm}
% p{2cm}
% p{2cm}
% p{1.15cm}
% p{2cm}
% p{3cm}
% p{2cm}
% p{5cm}
% p{1cm}
% p{1.1cm}||
% p{4cm}
% p{4cm}
% p{4cm}}
% \hline
% \makecell{Ref.\\ (Year)} & \makecell{Dataset\\Owner} & \# of\newline Datasets & Devices & Sensors & \# of\newline Sensors & Position & Model & \# of Subjects [M/F] & Activities & \# of Activities & \makecell{In-Out\\ Door}& Annotation & Advantages & Limitations \\ \hline \hline
% \cite{alam2015mobeacon}\\ (2015)
% &Yes
% &1
% &Smartphone, BLE Beacons, Video
% &Accelerometer, Gyroscope, RSSI
% &13
% &Smartphone in Front right pocket, Beacons on Objects and positions of a home environment
% &Semantic\newline  Knowledge
% &2[1/1]
% &Env. Context: Exercises bike, coach, dining table, bed, closets reading table, bookshelf, bathroom, kitchen, porch, 
% Low-level context: standing, walking, cycling, lying, sitting, 
% High-level exercising: exercising, preparing food, dining, watching tv, preparing clothes, studying, sleeping, bath rooming, cooking, past times, random.
% &25
% &Indoor
% &Annotate sensor data based on the recognized locaiton and used object
% &Reduces the labeling effort
% &Needs preliminary knowledge of the activity semantics and feedback from the user\\ \hline

% \cite{meurisch2015labels}\\ (2015)
% &Yes
% &1
% &Smartphone
% &accelerometer, location, light, proximity, gyroscope, loudness, wifi scans, smartphone usage, charging state, social network information, user-annotated human activity data
% &1
% &-
% &-
% &163
% &Provide a dataset for HAR
% &-
% &Indoor\newline Outdoor
% &Labeling is carried out manually through a smartphone app, there is some automatism: 
% 1) The data is pre-segmented by detecting a location change of the user. Each such segment needs to be labeled manually. 
% 2) there is a built-in metric of labeling quality (i.e., plausibility check, the time between event and label assignment, the time needed for labeling (too quick labeling cannot be thorough). It is rated positive when additional custom tags are assigned.
% &Provide a dataset 
% &Requires users interaction with the smartphone \\ \hline

% \cite{nino2016scalable}\\ (2016)
% &Yes
% &1
% &Video
% &Video
% &4
% &-
% &Poselet-based\newline  people detector
% &1
% &walking, eating, cooking, watching TV, reading, cleaning, using the laptop, lying down
% &8
% &Indoor
% &Recognize user position and interaction with the objects in the environment
% &Automatically annotates 80\% of the video frames with an accuracy of 99\%.
% &Works only with one person in the environment. Uses a pre-trained model to recognize the objects and measure distances in the environment\\ \hline

% \cite{cruciani2018personalized}\\ (2018)
% &Yes
% &1
% &Smartphone
% &Accelerometer, step counter, GPS
% &1
% &taurus pocket
% &\textit{na}
% &1
% &Sitting, Standing, Walking, Transportation
% &4
% &Indoor\newline Outdoor
% &Weak labels generation obtained through a heuristic as incombining Accelerometer and GPS data
% &overall accuracy of 87\% of a fully supervised approach against a 74\% with the proposed weakly supervised approach.
% &Requires users interaction with the smartphone \\ \hline

% \cite{cruz2019semi}\\ (2019)
% &Yes
% &1
% &Smartwatch
% &Accelerometer, Gyroscope, Audio
% &2
% &Wrist
% &Dynamic Time \newline Wrapping, SVM\newline  Sequential Minimal \newline Optimization (SMO)
% &15
% &hand gestures - recorded audio answers
% &36-20
% &Indoor
% &1 use the smartwatch to recognize specific hand gestures and position to annotate more complex activities, use a microphone to recognize specific home contexts and annotate the wearables data
% &Reduces the labeling effort
% &Requires preliminary annotated data for the hand gesture scenariou\\ \hline

% \cite{tonkin2019towards}\\ (2019)
% &Yes
% &1
% &Smartwatch, Environment
% &temperature, humidity, water usage, electricity usage per plug, and PIR sensor, accelerometer
% &\textit{na}
% &Enviroment and wrist
% &\textit{na}tural \newline Language \newline Toolkit’s 
% &1
% & Cooking-related activities: washing, chopping, cutting, peeling, mashing, grinding, percing, measuring, weighing
% &9
% &Indoor
% &Audio annotation of the start time of an activity
% &Easeier than the manually video-based annotaiton
% &Requires users interaction with the system\\ \hline

% \hline \hline
% \end{tabular}}
% \caption{Overview of Semi-automated hybrid methodologies.}\label{tab:S-H}
% \end{table}
% %\end{landscape}

%\begin{landscape}
\begin{table}[!th]
\centering
\caption{Semi-automated hybrid approaches.}\label{tab:S-H}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||cccccccccc}
\hline
\makecell{\textbf{Ref.}\\ \textbf{(Year)}} & \makecell{\textbf{Dataset}\\\textbf{Owner (\#)}} & \textbf{Devices} & \textbf{Sensors} & \makecell{\textbf{\# of}\\ \textbf{Sensors}} & \textbf{Position} & \textbf{Model} & \makecell{\textbf{\# of} \\\textbf{Subjects [M/F]}} & \textbf{Activities} & \makecell{\textbf{\# of} \\\textbf{Activities}} & \makecell{\textbf{In-Out}\\ \textbf{Door}}\\ \hline \hline
\makecell{\cite{alam2015mobeacon}\\ (2015)}
&yes (1)
&\makecell{smartphone,\\ BLE beacons,\\ video}
&\makecell{accelerometer,\\ gyroscope,\\ RSSI}
&13
&\makecell{smartphone in front\\ right pocket, beacons on\\ objects and positions \\of a home environment}
&\makecell{Semantic\\  Knowledge}
&2[1/1]
% &\makecell{Env. Context: Exercises bike,\\ coach, dining table, bed,\\ closets reading table, bookshelf,\\ bathroom, kitchen, porch,\\ 
% Low-level context: standing, walking,\\ cycling, lying, sitting,\\ 
% High-level exercising: exercising,\\ preparing food, dining,\\ watching tv, preparing clothes, studying,\\ sleeping, bath rooming, cooking,\\ past times, random.}
&\makecell{BHA, OBI, ADL}
&25
&Indoor
\\ \hline

\makecell{\cite{meurisch2015labels}\\ (2015)}
&yes (1)
&smartphone
&\makecell{accelerometer, location, light,\\ proximity, gyroscope, loudness,\\ wifi scans, smartphone usage, charging\\ state, social network information,\\ user-annotated human activity data}
&1
&-
&-
&163
&Provide a dataset for HAR
&-
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{nino2016scalable}\\ (2016)}
&yes (1)
&video
&video
&4
&-
&\makecell{Poselet-based\\  people detector}
&1
% &\makecell{walking, eating, cooking, watching TV,\\ reading, cleaning, using the laptop,\\ lying down}
&\makecell{BHA, OBI}
&8
&indoor\\ \hline

\makecell{\cite{cruciani2018personalized}\\ (2018)}
&yes (1)
&smartphone
&accelerometer, step counter, GPS
&1
&taurus pocket
&\textit{na}
&1
% &\makecell{Sitting, Standing,\\ Walking, Transportation}
&\makecell{BHA}
&4
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{cruz2019semi}\\ (2019)}
&yes (1)
&smartwatch
&\makecell{accelerometer,\\ gyroscope,\\ audio}
&2
&Wrist
&\makecell{Dynamic Time Warping,\\ SVM,  Sequential Minimal\\ Optimization (SMO)}
&15
&\makecell{hand gestures\\ - recorded audio answers}
&36-20
&indoor\\ \hline

\makecell{\cite{tonkin2019towards}\\ (2019)}
&yes (1)
&\makecell{smartwatch,\\ environment}
&\makecell{temperature, humidity,\\ water usage, electricity\\ usage per plug, and\\ PIR sensor, accelerometer}
&\textit{na}
&enviroment and wrist
&\makecell{Natural Language\\ Toolkit’s} 
&1
% &\makecell{Cooking-related activities:\\ washing, chopping, cutting,\\ peeling, mashing, grinding,\\ percing, measuring, weighing}
&\makecell{ADL, OBI}
&9
&indoor\\ \hline \hline 
\multicolumn{11}{c}{"-" in Columns Devices, \# of Sensors, Position, \# of Subjects [M/F], Activities, and \# of Activities separates the info of the different datasets.}
\end{tabular}}
\end{table}
%\end{landscape}

%\begin{landscape}
\begin{table}[!th]
\centering
\caption{Annotation method, Advantage's, and Limitations of Semi-automated hybrid approaches.}\label{tab:S-H-1}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||p{8cm}p{6cm}p{6cm}}
\hline
\textbf{Ref. (Year)} & \textbf{Annotation} & \textbf{Advantages} & \textbf{Limitations} \\ \hline \hline
\makecell{\cite{alam2015mobeacon}\\ (2015)}
& Annotates sensor data based on recognized location and used objects.
& Reduces labeling effort.
& Requires preliminary knowledge of activity semantics and user feedback.\\ \hline

\makecell{\cite{meurisch2015labels}\\ (2015)}
& Manual labeling through a smartphone app with some automation:
1) Pre-segmentation of data based on location change, requiring manual labeling of each segment.
2) Quality metrics for labeling with additional custom tags.
& Provides a dataset.
& Requires user interaction with the smartphone.\\ \hline

\makecell{\cite{nino2016scalable}\\ (2016)}
& Recognizes user positions and interaction with objects in the environment.
& Automatically annotates 80\% of the video frames with 99\% accuracy.
& Works only with one person in the environment. Relies on a pre-trained model for object recognition and distance measurement.\\ \hline

\makecell{\cite{cruciani2018personalized}\\ (2018)}
& Generates weak labels through a heuristic combining accelerometer and GPS data.
& Achieves an overall accuracy of 87\% compared to 74\% with fully supervised approaches.
& Requires user interaction with the smartphone.\\ \hline

\makecell{\cite{cruz2019semi}\\ (2019)}
& Uses a smartwatch to recognize hand gestures and the position for annotating complex activities, and a microphone to recognize specific home contexts and to annotate data from wearables.
& Reduces labeling effort.
& Requires preliminary annotated data for hand gesture scenarios.\\ \hline

\makecell{\cite{tonkin2019towards}\\ (2019)}
& Audio annotation of the start time of an activity.
& Easier than manual video-based annotation.
& Requires user interaction with the system.\\ \hline \hline
\end{tabular}}
\end{table}
%\end{landscape}


On such aim, in \cite{alam2015mobeacon}, the authors propose Mobeacon: a mobile phone and iBeacon sensor-based smart home activity recognition system, which uses Bagging Ensemble Learning (BEL) and Packaged Naive Bayes (PNB) classification algorithms for high-level activity recognition on smartphones. The author's goal is to incorporate the semantic knowledge of the testing environment and use it with the built-in adaptive learning models on the smartphone to ease the ground truth data annotation. They demonstrate that Mobeacon outperforms existing lightweight activity recognition techniques in terms of accuracy (max. 94\%) in a low-resource setting and is substantially efficient to reside on smartphones for recognizing ADLs in real-time. The authors also design an effective smartphone application interface for defining and creating an initial semantic knowledge base about the smart home environment and use their semantic knowledge base, expression tree-based activity construction, and inference cache to accelerate the activity recognition process of their lightweight BEL-based approach. %They show that their proposed BEL attests to the promise of their methodologies and outperforms several existing lightweight classifiers in terms of CPU, memory, cache occupancy and power consumption performance. They also demonstrate that their efficient duration model-based high-level activity merging provides higher accuracy in high-level activity recognition even with less accurate low-level activity detection.

Following, Meurisch et al. \cite{meurisch2015labels} proposed "Labels," a self-tracking mobile application that provides a user interface for annotating automatically collected sensor data from mobile, desktop, and social media platforms with metadata, such as performed activities. The study evaluated Labels with 163 participants over a four-week field study, collecting over 43,000 manually annotated data. Results show that participants annotated about 82.5\% of their place-related time slots with their performed activities. 
% The resulting human activities comprise physical and virtual sensor data, social network information, and user-annotated human activity data. The authors plan to use this dataset to recognize student activities using supervised machine learning approaches and enhance and use their tracking tools in field studies to better understand human behavior. They also plan to share their tools and collaborate with the community. 

Nino et al. \cite{nino2016scalable} presented a methodology for semi-automatic generation of reliable position annotations to evaluate multi-camera people-trackers on large video data sets. The methodology automatically computed most of the annotation data by recognizing the person's position and interaction with daily life objects. 
% For a small subset of data with insufficient reliability, an annotator verified the annotation by a simple binary decision task, which is faster than marking the correct person position. 
The proposed framework is generic and can handle additional trackers. 
The authors provided guidelines on applying the proposed methodology to new data sets and presented an exploratory study for the multi-target case. 
% The proposed method demonstrated scalability in semi-automatic annotation for long multi-camera sequences for the first time. The authors also estimated the precision of the resulting semi-automatically annotated data set, under given values of desired accuracy. Finally, the authors provided the annotated data set itself, which is available in two versions: the first version results from the proposed procedure, and the second from the exhaustive inspection to create ground truth. The authors hope that these annotated sequences will be useful to the research community since annotated multi-camera data sets of such length are not yet reported in literature.

In their work, Cruciani et al. \cite{cruciani2018personalized} proposed an annotation system that combines two information sources: GPS and a step counter. The GPS data provides valuable information for discriminating between activities based on their position and estimated speed and labeling such activities based on defined heuristics. For example, Walking, running, and transportation activities can be differentiated using the speed ranges associated with each activity (e.g., walking: 1.4 - 2.0 m/s, running: 3.0 - 6.0 m/s, transportation: > 8 m/s). To refine the labeling and reduce mislabeled samples, the system incorporates a step counter. 
The system combines the GPS and step counter data in a rule-based intersection of the information sources. This combination allows for more accurate labeling and discrimination between activities. For example, it can differentiate between running and driving in traffic, or detect running activities at the gym that may not be detectable using GPS alone.

In \cite{cruz2019semi}, the authors proposed two novel approaches for semi-automated online data labeling. The first approach is based on the recognition of subtle finger gestures performed in response to a data-labeling query. In contrast, the second approach focuses on labeling activities that have an auditory manifestation and uses a classifier to have an initial estimation of the activity and a conversational agent to ask the participant for clarification or additional data. Results show that while both studies have limitations, they achieve 80\% to 90\% precision. In addition, the authors described an approach for the semi-automatic labeling of environmental audio data, and presented results of experiments to assess its feasibility. 

In \cite{tonkin2019towards}, the authors proposed a participant-centric free-text annotation process to facilitate activity recognition in the kitchen environment and characterized the resulting annotations. They reviewed the data from the study to establish the feasibility of implementing cooking complexity metrics within the dataset, and found that the annotations explored in the paper constitute a useful basis for exploratory analysis of the data. 
However, they noted that the granularity of the annotations is not optimal for certain tasks and may benefit from a more detailed set of annotations. The authors also identified several features of meal preparation complexity that are readily detectable within their sensor data, including monitored appliance use, water use, and the energy released as heat and humidity released during the task. 
% They suggested that the most straightforward definition of cooking or meal complexity to apply in the context of their dataset is cooking complexity, followed by the facets of meal preparation complexity that are most readily detectable within their sensor data. Lastly, the authors discussed their ongoing research, which includes the development and evaluation of several feature detectors and the exploration of changes in behavior using a companion dataset of post-operative patients over several months.

% \newpage
\subsection{Fully automated}\label{sec:4.2}
In this section, we categorize the 14 papers on fully-automated data annotation techniques for HAR into the three previously mentioned categories and provide detailed descriptions of their proposed methods and key features. Table \ref{tab:all-papers} demonstrates that none of the selected papers focus on hybrid fully-automated methodologies. Therefore, this section will focus solely on data-centric and environment-based methods. 

\subsubsection{Data Centric-based}\label{sec:4.2.1}
These studies propose innovative fully-automated data-centric methodologies for HAR, utilizing various techniques, including active learning, automatic labeling algorithms, and unsupervised learning. 
These methodologies strive to minimize the manual effort and cost associated with annotating large datasets while enhancing the accuracy and performance of activity recognition models. By integrating human expertise with automated processes, these approaches offer efficient and effective solutions for labeling and analyzing human activities in diverse contexts and settings. 
Tables \ref{tab:H-DD} and \ref{tab:H-DD-1} provides an overview of the methodologies falling into such category. 

%\begin{landscape}
% \begin{table}[!th]
% \centering
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c||c
% p{1.1cm}
% p{2cm}
% p{2cm}
% p{1.15cm}
% p{2cm}
% p{3cm}
% p{2cm}
% p{5cm}
% p{1cm}
% p{1.1cm}||
% p{4cm}
% p{4cm}
% p{4cm}}
% \hline
% \makecell{Ref.\\ (Year)} & \makecell{Dataset\\Owner} & \# of\newline Datasets & Devices & Sensors & \# of\newline Sensors & Position & Model & \# of Subjects [M/F] & Activities & \# of Activities & \makecell{In-Out\\ Door}& Annotation & Advantages & Limitations \\ \hline \hline
% \cite{jardim2016automatic}\\ (2016)
% &Yes
% &1
% &Kinect
% &Depth image
% &1
% &-
% &Segmentation \newline and Temporal \newline Clustering
% &12
% &rightleft punch, frontside right kick, frontside left kick, back fist, elbow strike
% &8
% &Indoor
% &Extract features related to bodys joints and use the knowledge on the performed activity to recognize it and automatically label such activity. 
% &Fully automated
% &Reduced set of recognized activities. Not easy to scale towards other activities.\\ \hline

% \cite{rokni2018autonomous}\\ (2018)
% &Yes
% &1
% &Xsens MTx
% &Accelerometer, Gyroscope, Magnetometer
% &5
% &Torso, Right Arm, Left Arm, Right Leg, Left Leg
% &Transfer \newline Learning
% &8[4/4]
% &sitting, standing, lying, ascending descending stairs, in elevator, walking, running, exercising on a stepper, exercising on a cross trainer, cycling 1, cycling 2, rowing, jumping, playing basketball
% &15
% &Indoor\newline Outdoor
% &Synchronous Multi-view Learning starts consist of (a) labeling target instances by semi-labels Minimum-Error Exact Labeling (MEEL) and continue with (b) clustering target
% instances. (c) A weighted bipartite graph is built on clusters and activities, and after finding the best assignment, and (d) cluster labels are
% propagated to their instances.
% &Does not require user feedback and achieves a recogniton accuracy of 84\% on unlabeled data. 
% &Accuracy lower than on labeled data. \\ \hline

% \cite{liang2018automatic}\\ (2018)
% &Yes
% &1
% &STM32F103R IMU
% &Accelerometer, Gyroscope
% &9
% &left upper arm, right upper arm, left wrist, right wrist, front waist, left thigh, right thigh, left ankle, and right ankle
% &
% &6[5/1]
% &standing still, sitting, lying down, walking, ascending, and descending stairs,  jumping up and down, and squatting slowly and quickly, fall forward, fall backwards), fall to the left, and fall to the right
% &17
% &Indoor
% &Automatic labeling based on mathematical transformation to detect activity endpoints performed in three steps: i) preliminary segmentation, ii) endpoint detection, and iii) labels assignment.
% &Does not requires feedbacks from the users and achieves an recogniton accuracy of 89\% on unlabeled data. 
% &Reduced set of recognized activities. Not easy to scale towards other activities. \\ \hline

% \cite{zhang2020deep}\\ (2020)
% &No
% &3
% &Video, IMU
% &Video, Accelerometer, Gyroscope
% &5
% &arms, legs and back
% &conditional VARiational AutoEncoder (cVAE)\newline conditional Generative Adversarial Network (cGAN)
% &100
% &Eating,  ADL
% &\textit{na}
% &Indoor\newline Outdoor
% &Use video - sensors dataset to train the model and generate synthetic data for the studied activities. 
% &Genertates synthetic motion data of specific activities from videos
% &No accuracy of the system is provided\\ \hline

% \cite{jeng2021wrist}\\ (2021)
% &Yes
% &1
% &Koala IMU
% &Accelerometer
% &2
% &Wrist, Chest
% &Knowledge based 
% &2
% &Sleeping posture
% &4
% &Indoor
% &Use a chest-mounted accelerometer to annotate the sleeping and not-sleeping postures.
% &Data annotation is fully automatized 
% &\textit{na}\\ \hline

% \cite{ullrich2021detection}\\ (2021)
% &Yes
% &1
% &Mobile GaitLab IMU
% &Accelerometer, Gyroscope
% &2
% &Insoles
% &Knowledge based 
% &12[10/2]
% &Gait phases
% &\textit{na}
% &Indoor\newline Outdoor
% &Knowledge-based
% &Acheived 94 F1-score in the recognition. 
% &\textit{na}\\ \hline

% \cite{ma2021unsupervised}\\ (2021)
% &No
% &3
% &Smartwatch, Smartphone - Smartphone - Smartphone
% &Accelerometer, Gyroscope
% &2 - 1 - 1
% &Pocket, wrist - pocket - pocket
% &CNN-BiLSTM \newline Autoencoder, \newline  k-Means
% &36 - 66 - 24
% &biking, sitting, standing, walking, climbStair-up,
% and climbStair-down - 4 falls, 11 ADLs - walking, jogging,
% going downstairs, going upstairs, sitting and standing
% &6 - 15 - 6
% &Indoor
% &Unsupervised learning through Multi-task deep clustering
% &Achive an average F1-Score higher of 85\%.
% &Less performant then supervised techniques. \\ \hline

% \cite{qi2022dcnn}\\ (2022)
% &Yes
% &1
% &Smartphone, Kinect
% &Accelerometer, Gyroscope, Magnetometer, Depth Image
% &2
% &Arm, 25 Body Joints
% &Hierarchical\newline  k-Medoids 
% &10[6/4]
% &walk, twist, squats, lunge, jump rope, jump jack, jog, jab cross, raise, standLeg, standHand, stand
% &12
% &Indoor
% &Unsupervised learning through Hierarchical k-Medoids 
% &Achieves an accuracy of 93,89\% in labeling
% &\textit{na}\\ \hline

% \cite{lin2022clustering}\\ (2022)
% &No
% &1
% &Smartphone
% &Accelerometer, Gyroscope
% &1
% &Waist
% &Feature Selection based on Fuzzy C-means Particle Swarm Optimization (FS-FCPSO)
% &30
% &walking, sitting, standing, upstairs,
% downstairs, and lying down
% &6
% &Indoor
% &Unsupervised learning
% &Perfromes better than a classic k-Means algorithm. 
% &Less performant than supervised techniques. \\ \hline

% \hline \hline
% \end{tabular}}
% \caption{Overview of Fully-automated data-driven based methodologies.}\label{tab:H-DD}
% \end{table}
%\end{landscape}

\begin{table}[!th]
\centering
\caption{Fully-automated data-driven based approaches.}\label{tab:H-DD}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||c
ccccccccc}
\hline
\makecell{\textbf{Ref.}\\ \textbf{(Year)}} & \makecell{\textbf{Dataset}\\\textbf{Owner (\#)}} & \textbf{Devices} & \textbf{Sensors} & \makecell{\textbf{\# of}\\ \textbf{Sensors}} & \textbf{Position} & \textbf{Model} & \makecell{\textbf{\# of} \\\textbf{Subjects [M/F]}} & \textbf{Activities} & \makecell{\textbf{\# of} \\\textbf{Activities}} & \makecell{\textbf{In-Out}\\ \textbf{Door}}\\ \hline \hline
\makecell{\cite{jardim2016automatic}\\ (2016)}
&yes (1)
&kinect
&\makecell{depth\\ image}
&1
&-
&\makecell{Segmentation\\ and Temporal\\ Clustering}
&12
% &\makecell{rightleft punch,\\ frontside right kick,\\ frontside left kick,\\ back fist,\\ elbow strike}
&\makecell{PA}
&8
&indoor\\ \hline

\makecell{\cite{rokni2018autonomous}\\ (2018)}
&yes (1)
&\makecell{Xsens\\ MTx}
&\makecell{accelerometer,\\ gyroscope,\\ magnetometer}
&5
&\makecell{torso, right arm,\\ left arm, right leg,\\ left leg}
&\makecell{Transfer\\ Learning}
&8[4/4]
% &\makecell{sitting, standing, lying,\\ ascending descending stairs,\\ in elevator, walking, running,\\ exercising on a stepper,\\ exercising on a cross trainer,\\ cycling 1, cycling 2, rowing,\\ jumping, playing basketball}
&\makecell{BHA}
&15
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{liang2018automatic}\\ (2018)}
&yes (1)
&IMU
&\makecell{accelerometer,\\ gyroscope}
&9
&\makecell{left upper arm,\\ right upper arm,\\ left wrist, right wrist,\\ front waist, left thigh,\\ right thigh, left ankle,\\ and right ankle}
&
&6[5/1]
% &\makecell{standing still, sitting, lying down,\\ walking, ascending, and descending stairs,\\  jumping up and down, and squatting slowly\\ and quickly, fall forward, fall backwards,\\ fall to the left, and fall to the right}
&\makecell{BHA, R}
&17
&indoor\\ \hline

\makecell{\cite{zhang2020deep}\\ (2020)}
&no (3)
&video, IMU
&\makecell{video,\\ accelerometer,\\ gyroscope}
&5
&\makecell{arms, legs\\ and back}
&\makecell{conditional VARiational\\ AutoEncoder (cVAE)\\ conditional Generative\\ Adversarial Network (cGAN)}
&100
% &Eating,  ADL
&\makecell{ADL}
&\textit{na}
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{jeng2021wrist}\\ (2021)}
&yes (1)
&IMU
&accelerometer
&2
&\makecell{wrist,\\ chest}
&\makecell{Knowledge\\ based} 
&2
&\makecell{Sleeping\\ posture}
&4
&indoor\\ \hline

\makecell{\cite{ullrich2021detection}\\ (2021)}
&yes (1)
&IMU
&\makecell{accelerometer,\\ gyroscope}
&2
&insoles
&\makecell{Knowledge\\ based} 
&12[10/2]
&\makecell{Gait\\ phases}
&\textit{na}
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{ma2021unsupervised}\\ (2021)}
&no (3)
&\makecell{smartwatch,\\ smartphone\\ - smartphone\\ - smartphone}
&\makecell{accelerometer,\\ gyroscope}
&\makecell{2 - 1\\ - 1}
&\makecell{pocket, wrist\\ - pocket\\ - pocket}
&\makecell{CNN-BiLSTM\\ Autoencoder,\\ k-Means}
&36 - 66 - 24
% &\makecell{biking, sitting, standing, walking, ascending stairs,\\
% descending stairs - 4 falls, 11 ADLs - walking,\\ jogging, going downstairs, going upstairs,\\ sitting and standing}
&\makecell{BHA, ADL, R}
&6 - 15 - 6
&Indoor \\ \hline

\makecell{\cite{qi2022dcnn}\\ (2022)}
&yes (1)
&\makecell{smartphone,\\ kinect}
&\makecell{accelerometer,\\ gyroscope,\\ magnetometer,\\ depth image}
&2
&\makecell{arm, 25\\ body joints}
&\makecell{Hierarchical\\ k-Medoids} 
&10[6/4]
% &\makecell{walk, twist, squats, lunge,\\ jump rope, jump jack, jog, jab cross,\\ raise, standLeg, standHand, stand}
&\makecell{BHA, PA}
&12
&indoor\\ \hline

\makecell{\cite{lin2022clustering}\\ (2022)}
&no (1)
&smartphone
&\makecell{accelerometer,\\ gyroscope}
&1
&Waist
&\makecell{Feature Selection based\\ on Fuzzy C-means Particle\\ Swarm Optimization\\ (FS-FCPSO)}
&30
% &\makecell{walking, sitting, standing,\\ upstairs,
% downstairs, and lying down}
&\makecell{BHA}
&6
&indoor\\ \hline \hline
\multicolumn{11}{c}{"-" in Columns Devices, \# of Sensors, Position, \# of Subjects [M/F], Activities, and \# of Activities separates the info of the different datasets.}
\end{tabular}}
\end{table}


\begin{table}[!th]
\centering
\caption{Annotation method, Advantages, and Limitations of Fully-automated data-driven based approaches.}\label{tab:H-DD-1}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||
p{8cm}
p{6cm}
p{6cm}}
\hline
\textbf{Ref. (Year)} & \textbf{Annotation} & \textbf{Advantages} & \textbf{Limitations} \\ \hline \hline
\makecell{\cite{jardim2016automatic}\\ (2016)}
& Extracts features related to body joints and utilizes knowledge of performed activities to automatically recognize and label them.
& Fully automated.
& Limited set of recognized activities. Difficulty in scaling to other activities. \\ \hline

\makecell{\cite{rokni2018autonomous}\\ (2018)}
& Utilizes Synchronous Multi-view Learning, including labeling target instances by semi-labels Minimum-Error Exact Labeling (MEEL), clustering target instances, building a weighted bipartite graph, and propagating cluster labels to their instances.
& Does not require user feedback and achieves a recognition accuracy of 84\% on unlabeled data.
& Lower accuracy compared to labeled data. \\ \hline

\makecell{\cite{liang2018automatic}\\ (2018)}
& Automatically labels activities based on mathematical transformations for detecting activity endpoints, performed in three steps: preliminary segmentation, endpoint detection, and label assignment.
& Does not require user feedback and achieves a recognition accuracy of 89\% on unlabeled data.
& Limited set of recognized activities. Difficulty in scaling to other activities. \\ \hline

\makecell{\cite{zhang2020deep}\\ (2020)}
& Uses a video-sensors dataset to train the model and generate synthetic data for the studied activities.
& Generates synthetic motion data of specific activities from videos.
& No system accuracy is provided. \\ \hline

\makecell{\cite{jeng2021wrist}\\ (2021)}
& Utilizes a chest-mounted accelerometer to annotate sleeping and non-sleeping postures.
& Data annotation is fully automated.
& Sleeping specific. \\ \hline

\makecell{\cite{ullrich2021detection}\\ (2021)}
& Knowledge-based annotation.
& Achieves a 94\% F1-score in recognition.
& Knowledge-based. \\ \hline

\makecell{\cite{ma2021unsupervised}\\ (2021)}
& Utilizes unsupervised learning through Multi-task deep clustering.
& Achieves an average F1-Score higher than 85\%.
& Less performant than supervised techniques. \\ \hline

\makecell{\cite{qi2022dcnn}\\ (2022)}
& Utilizes unsupervised learning through Hierarchical k-Medoids.
& Achieves an accuracy of 94\% in labeling.
& - \\ \hline

\makecell{\cite{lin2022clustering}\\ (2022)}
& Utilizes unsupervised learning.
& Performs better than the classic k-Means algorithm.
& Less performant than supervised techniques. \\ \hline \hline

\end{tabular}}
\end{table}

The initial study that introduced fully-automatic data-centric annotation techniques for HAR was conducted by Jardim et al. in \cite{jardim2016automatic}. The researchers proposed a method for recognizing human actions from a continuous sequence of actions captured by a Kinect sensor. They suggested employing an automatic temporal segmentation approach to divide the sequence into individual actions, employing a straightforward filtering technique based on joint movement. Furthermore, they presented an automatic labeling method for human actions by utilizing a clustering algorithm on a subset of available features. Jardim et al. described a novel dataset comprising action sequences recorded with Kinect and assessed their proposed method using k-means clustering. They observed that the clustering algorithm's performance was influenced by the choice of features and neighboring actions. To enhance the outcomes, they recommended the utilization of Euler angles and Dynamic Time Warping (DTW) techniques. The authors successfully demonstrated that combining clustering and filtering techniques enables unsupervised labeling of human actions captured by a depth-sensing camera that tracks skeleton key-points.

In their publication, Rokni et al. \cite{rokni2018autonomous} introduced a novel approach called autonomous multi-view learning, capable of dynamically retraining machine learning algorithms in real time without the need for labeled training data. This approach can be applied in both online and batch modes. 
%The authors assessed the inherent correlation between observations from an existing sensor view with trained algorithms and a new sensor view that requires algorithm development. 
By employing autonomous multi-view learning in batch mode, they achieved an 83.7\% accuracy in activity recognition, representing a 9.3\% improvement facilitated by automatic data labeling in the new sensor node. Additionally, the online learning algorithm achieved an 82.2\% accuracy in activity recognition. 
This study represents an initial step towards developing next-generation wearables that possess computational autonomy and can automatically learn machine learning algorithms. 
% Ongoing research focuses on creating transfer learning algorithms that address the dynamically evolving behavior of human-centered monitoring applications. The authors also highlighted the potential for future work in expanding activity recognition capabilities to encompass new, unseen activities, where approaches like active learning could minimize the need for queries to external knowledge sources.

The paper from Liang et al. \cite{liang2018automatic} presents ALF, an Automatic Labeling Framework for in-laboratory settings HAR, eliminating the need for a small initial set of labeled data. The proposed framework converts time series activity data into absolute wavelet energy entropy and detects activity endpoints using constraints and information extracted from a predefined Human Activity Sequence (HAS). 
The authors evaluated the framework's performance on a collected dataset and the UCI HAR Dataset\cite{anguita2013public}, achieving average precision and recall scores above 81.9\% and average F-measure scores above 88.9\%. The ALF framework significantly reduces labeling efforts while maintaining labeling accuracy. It provides a fast and reliable method for generating labeled datasets, with a total labeling time of approximately 18.6 minutes, which is 75.8\% shorter than the average manual labeling time of 76.8 minutes.


In their publication \cite{zhang2020deep}, Zhang et al. addressed the issue of limited labeled datasets for activity recognition using wearable sensors. They proposed two deep generative cross-modal architectures to synthesize accelerometer data streams from video data streams. The approach utilizes a conditional Generative Adversarial Network (cGAN) to generate sensor data based on video data and incorporates a conditional Variational AutoEncoder (cVAE)-cGAN to further enhance data representation. 
The proposed method was evaluated through experiments on publicly available sensor-based activity recognition datasets, comparing models trained on synthetic data against those trained on real sensor data. 
%The anticipated contributions of this research include the development of two end-to-end deep cross-modal models for generating accelerometer data from video, evaluation through experiments on multiple datasets, and the establishment of a latent representation space for sensor data conditioned on video, enabling other video-sensor-based multimodal tasks. 
This work aims to expand the availability of labeled on-body sensor data by generating synthetic data from videos, providing the research community with techniques to transfer labels from video to on-body sensors. This, in turn, unlocks a broader range of applications in activity analysis. 

In their publication \cite{jeng2021wrist}, Jeng et al. introduced iSleePost, an easy-to-use intelligent sleep posture monitoring system for home care. Instead of manual labeling, iSleePost automatically recognizes body posture to label the data. By analyzing data from a single wrist sensor, the system achieves an accuracy of up to 85\% in posture recognition. 
The authors evaluated two different learning algorithms, with the random forest algorithm achieving over 70\% accuracy and the SVM algorithm achieving 73\% accuracy. iSleePost is more cost-effective compared to existing approaches that rely on pressure mats, cameras, or specialized equipment. 
The authors successfully demonstrated the system's ability to accurately monitor sleep postures using only a wrist accelerometer, providing valuable insights for the design of health monitoring systems. 
% This research paves the way for potential future investigations in areas such as elder healthcare and adjusting medicine dosages based on sleep posture profiles. 

In their publication \cite{ullrich2021detection}, the authors introduced a novel algorithmic pipeline for the automated detection of unsupervised standardized gait tests from continuous real-world IMU data. This pipeline addresses potential errors caused by patient-system interaction during unsupervised gait tests. The proposed approach involves gait sequence detection, peak enhancement, and subsequence DTW to identify gait test series, which are further decomposed into individual 4 x 10 Meters-Walking-Tests based on walking speed. The algorithm was evaluated using 419 available gait test series, achieving an F1-score of 88.9\% for detection and 94.0\% for decomposition. 
% This study contributes to improved automated processing of real-world IMU gait data, facilitating the seamless integration of standardized tests into continuous long-term recordings. 
% However, it should be noted that the evaluation of gait test series decomposition was limited to those with three subsequent 4×10MWTs, and the detection of other gait tests or shorter tests like TUG may require more advanced techniques. 
% Future research should explore the detection of various gait tests by considering more complex machine learning methods.
% Additionally, the presented algorithm, which focuses on turnings, may also be applicable in single-sensor settings involving a gyroscope, necessitating further investigation.
% The algorithm provides a reliable tool for clinicians and patients in recording and processing the required data, with potential applications in other diseases characterized by motor impairments. 
% This study represents a significant advancement in real-world gait analysis, facilitating further clinical research to better understand and treat movement disorders.

In \cite{ma2021unsupervised}, Ma et al., presented an unsupervised automatic annotation technique in HAR, without the need for domain knowledge or manual data annotation. 
The proposed approach is an end-to-end multi-task deep clustering framework that integrates feature representation, clustering, and classification tasks into a uniform learning framework. The framework comprises an autoencoder neural network structure to extract features from the raw signals and form compressed latent feature representation, a K-means clustering algorithm to partition the unlabeled dataset into groups to produce pseudo labels for the instances, and a DNN classifier to train the human activity classification model based on the latent features and pseudo labels. The authors conducted extensive experiments based on three publicly available datasets showing that the proposed approach outperforms existing clustering methods under completely unsupervised conditions and achieves performance similar to full-supervised learning when retraining the extracted latent feature representation. 
%The authors also discussed the future works of expanding the proposed model to help experts in fields with unlabeled data discover behavior classes, such as studying animal communication, zero resource speech recognition, tracking wild animal activities, and studying human behavior patterns and mental healthiness based on smartphone sensing data. The proposed approach significantly reduces human-based data annotation costs and narrows the gap between unsupervised and supervised HAR. 

In \cite{qi2022dcnn}, Qi et al. proposed a novel framework for smartphone-based HAR that uses depth data to guide the labeling process. 
The framework combines data from the Microsoft Kinect camera and the smartphone's IMU signals to identify 12 complex daily activities. The proposed framework comprises five clustering layers and a deep learning-based classification model. The authors employed a Hierarchical k-medoids (Hk-medoids) algorithm to obtain labels with high accuracy. 
Additionally, the performance of the Deep Convolutional Neural Network (DCNN) classification model was evaluated and compared to other machine learning and deep learning methods. Although the proposed framework opens up new opportunities for human-computer interaction and intelligence learning, the authors acknowledge the need for improved labeling accuracy in future work. They proposed a calibration approach to mitigate the effect of artifact and drifting noises on the obtained 3D joints data.

Finally, Lin et al. \cite{lin2022clustering} to improve the accuracy of automatic labeling in HAR applied the feature selection based on Fuzzy C-means Particle Swarm Optimization (FS-FCPSO) to mark six human activities automatically, including walking, sitting, standing, upstairs, downstairs, and lying down. 
The results of this method were compared with those of K-means and fuzzy C-means algorithms. The authors used a data set that included 30 volunteers aged 19 - 48 and captured the 3-axis linear acceleration and 3-axis angular velocity using a Samsung Galaxy S II phone with an embedded accelerometer and gyroscope. 
The feature vector of each window was obtained from calculation variables in the time domain and frequency domain. 
The FS-FCPSO method was more suitable for automatic labeling in HAR than K-means and fuzzy C-means algorithms. 
The contribution of this research was to adopt the feature selection method based on fuzzy C-average particle swarm optimization to improve the accuracy of automatic labeling results. 
The authors reduced 561 feature points to 163 features as a cluster subset and proved that feature selection based on binary PSO could effectively enhance the application of the fuzzy C-means clustering method in HAR automatic labeling.



\subsubsection{Environment-based}\label{sec:4.2.2}
This section concludes the description of the categories introduced by the taxonomy of Figure \ref{fig:tax_2} discussing methodologies presenting fully automated environment-based techniques in HAR. Tables \ref{tab:H-ED} and \ref{tab:H-ED-1} offers a comprehensive summary of the articles included in the Fully-automated Environment-based category of automatic annotation systems in HAR.

%\begin{landscape}
% \begin{table}[!th]
% \centering
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c||c
% p{1.1cm}
% p{2cm}
% p{2cm}
% p{1.15cm}
% p{2cm}
% p{3cm}
% p{2cm}
% p{5cm}
% p{1cm}
% p{1.1cm}||
% p{4cm}
% p{4cm}
% p{4cm}}
% \hline
% \makecell{Ref.\\ (Year)} & \makecell{Dataset\\Owner} & \# of\newline Datasets & Devices & Sensors & \# of\newline Sensors & Position & Model & \# of Subjects [M/F] & Activities & \# of Activities & \makecell{In-Out\\ Door}& Annotation & Advantages & Limitations \\ \hline \hline
% \cite{loseto2013mining}\\ (2013)
% &Yes
% &1
% &Smartphone, Mobile APP
% &Accelerometer, GPS, Mobile APP
% &3
% &-
% &Semantic Web Language
% &1
% &home-office, office-bar, bar-office, office-gym, gym-office
% &5
% &Indoor\newline Outdoor
% &-
% &-
% &-\\ \hline

% \cite{al2017annotation}\\ (2017)
% &No
% &3
% & Enviromental
% & Accelerometer, Temperature, PIR
% &20 - 25 - 33
% &-
% &Hidden Markov \newline Model (HMM) and Conditional \newline Random Field (CRF) 
% &4 - 2 - 1
% &ADLs
% &16  - 10 - 15
% &Indoor
% &Probabilistic modeling of activites
% &No partecipants intervention is required.  Able to extract to also hidden activities/ehaviourse. 
% &The average annotaiton accuracy is 73 \%.
% \\ \hline

% \cite{demrozi2021towards}\\ (2021)
% &Yes
% &1
% &Smartwatch, BLE Beacons
% &Accelerometer, Gyroscope, Magnetometer, BLE antenna
% &2
% &Wrist, ODLs
% &Regression \newline models. 
% &1
% &-
% &-
% &Indoor
% &Recognize the distance between ODL's and Smartwatch through the study of RSSI. 
% &Fully automated
% &RSSI values a higly dependedet onf the enironment. \\ \hline

% \cite{dissanayake2021indolabel}\\ (2021)
% &Yes
% &1
% &ASUS ZenWatch3 smartwatch, Access Points
% &Accelerometer, Gyroscope, RSSI
% &36
% &Wrist, Environment AP
% &Location Specificity Measure and activity smililarity matrix calculation
% &4[3/1]
% &chop, wash dishes, wash hands, brush teeth, wash face, lie, use toilet paper,wash hands, eat, drink, sit, use PC, write on a notebook, smoke
% &14
% &Indoor
% &Predict the location of a room where a user was located by discovering location-specific sensor data motifs in sensor data from the user’s  smartwatch.
% &Achieves an F1-Score of 85\% in labeling activities
% &-\\ \hline

% \hline \hline
% \end{tabular}}
% \caption{Overview of Fully-automated environment-based methodologies.}\label{tab:H-ED}
% \end{table}
%\end{landscape}

\begin{table}[!th]
\centering
\caption{Fully-automated environment-based approaches.}\label{tab:H-ED}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||c
ccccccccc}
\hline
\makecell{\textbf{Ref.}\\ \textbf{(Year)}} & \makecell{\textbf{Dataset}\\\textbf{Owner (\#)}} & \textbf{Devices} & \textbf{Sensors} & \makecell{\textbf{\# of}\\ \textbf{Sensors}} & \textbf{Position} & \textbf{Model} & \makecell{\textbf{\# of} \\\textbf{Subjects [M/F]}} & \textbf{Activities} & \makecell{\textbf{\# of} \\\textbf{Activities}} & \makecell{\textbf{In-Out}\\ \textbf{Door}}\\ \hline \hline
\makecell{\cite{loseto2013mining}\\ (2013)}
&yes (1)
&\makecell{smartphone\\ mobile app}
&\makecell{accelerometer\\ GPS, mobile app}
&3
&-
&\makecell{Semantic Web\\ Language}
&1
% &\makecell{home-office, office-bar,\\ bar-office, office-gym, gym-office}
&\makecell{PA}
&5
&\makecell{indoor\\ outdoor}\\ \hline

\makecell{\cite{al2017annotation}\\ (2017)}
&no (3)
&enviromental
&\makecell{accelerometer,\\ temperature,\\ PIR}
&\makecell{20 - 25\\ - 33}
&-
&\makecell{Hidden Markov\\ Model (HMM) and\\ Conditional Random\\ Field (CRF)} 
&4 - 2 - 1
% &ADLs
&\makecell{ADL}
&16  - 10 - 15
&indoor\\ \hline

\makecell{\cite{demrozi2021towards}\\ (2021)}
&yes (1)
&\makecell{smartwatch,\\ BLE beacons}
&\makecell{accelerometer,\\ gyroscope,\\ magnetometer,\\ BLE antenna}
&2
&wrist, ODLs
&\makecell{Regression\\ models.} 
&1
&-
&-
&indoor\\ \hline

\makecell{\cite{dissanayake2021indolabel}\\ (2021)}
&yes (1)
&\makecell{smartwatch,\\ access points}
&\makecell{accelerometer,\\ gyroscope, RSSI}
&36
&\makecell{wrist,\\ environment AP}
&\makecell{Location Specificity\\ Measure and activity\\ similarity matrix\\ calculation}
&4[3/1]
% &\makecell{chop, wash dishes, wash hands\\, brush teeth, wash face, lie, use toilet\\ paper,wash hands, eat,\\ drink, sit, use PC,\\ write on a notebook, smoke}
&\makecell{ADL, OBI}
&14
&Indoor\\\hline \hline
\multicolumn{11}{c}{"-" in Columns \# of Sensors, Position, \# of Subjects [M/F], Activities, and \# of Activities separates the info of the different datasets.}
\end{tabular}}
\end{table}


\begin{table}[!th]
\centering
\caption{Annotation method, Advantages, and Limitations of Fully-automated environment-based approaches.}\label{tab:H-ED-1}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||
p{8cm}
p{6cm}
p{6cm}}
\hline
\textbf{Ref. (Year)} & \textbf{Annotation} & \textbf{Advantages} & \textbf{Limitations} \\ \hline \hline
\makecell{\cite{loseto2013mining}\\ (2013)}
&-
&-
&-\\ \hline

\makecell{\cite{al2017annotation}\\ (2017)}
& Probabilistic modeling of activities.
& No participant intervention required. Able to extract hidden activities/behaviors.
& Average annotation accuracy is 73\%. \\ \hline

\makecell{\cite{demrozi2021towards}\\ (2021)}
&Recognize the distance between ODL's and Smartwatch through the study of BLE signals. 
&Fully automated
&BLE signals highly dependent on the environment. \\ \hline

\makecell{\cite{dissanayake2021indolabel}\\ (2021)}
& Predicts the room location of a user by discovering location-specific sensor data motifs from the user's smartwatch.
& Achieves an F1-Score of 85\% in labeling activities.
& - \\ \hline \hline
\end{tabular}}
\end{table}


% In \cite{szewcyzk2009annotating}, 
The first approach proposed in such a category was presented by Loseto et al. in \cite{loseto2013mining}. 
The authors proposed an agent running over an Android mobile app that utilizes Semantic Web languages to perform automated profile annotation based on the data collected by embedded micro-devices, logs, and applications on a smartphone. 
The system annotates the data by using motion, location, and smartphone usage to annotate the user's activity automatically. The resulting semantic-based daily profile can be leveraged in an Ambient Intelligence scenario to adapt the environment to user preferences. The agent was designed and implemented as an Android application and tested in a case study, demonstrating its feasibility and effectiveness. 
%The authors suggested future work to include a more extensive experimental campaign involving multiple users, the assessment of battery drain and storage peaks, a comparison with existing approaches, and the integration of multimodal information for more precise user characterization.

In \cite{al2017annotation}, Al Zamil et al. proposed a methodology for automated data annotation in smart home environments, specifically for modeling activities based on spatially recognized actions and validating the assignment of labels through temporal relations. 
The proposed technique utilized Hidden Markov Models (HMM) and Conditional Random Field (CRF) model to detect segment labels accurately. 
The authors defined the segmentation problem as an optimization problem that minimizes ambiguity to improve overall accuracy. The experiments performed on CASAS data sets \cite{cook2009collecting} indicated that the proposed methodology achieved better performance than state-of-the-art methodologies, with contributions including the modeling of activity actions as states and transitions, the incorporation of spatial and temporal relationships, and the algorithmic segmentation of incoming actions. 
% This research presents an efficient solution for annotating activities in smart home environments, where performance, ambiguity, and concurrency are prevalent.

In the approach presented by Demrozi et al. \cite{demrozi2021towards}, the methodology involves mapping BLE beacons to the locations or objects where a human typically performs activities, such as cooking or working and associating the data collected by sensors embedded in the user's smartwatch to the nearest BLE beacon. This allows data from the smartwatch sensors to be automatically labeled with the human activity associated with the nearest beacon. 
The proposed methodology is low-cost and uses regression models to estimate the distance between the user and the beacons accurately. 
The methodology was found to estimate the distance between emitters and receivers with an RMSE of 13 cm and an MAE of 10 cm. The outcome is an automatically-annotated dataset that can be used to design dedicated HAR models. 
%Future work will aim to validate the proposed methodology through video recordings and compare the labeling obtained by this method to state-of-the-art video-based data annotation methods.

Finally, in \cite{dissanayake2021indolabel}, Dissanayake et al. present IndoLabel, a method to automatically detect short sensor data motifs specific to a location class, and builds an environment-independent location classifier without requiring handcrafted rules and templates. 
The authors believe that this method can be utilized to extract class-specific sensor data segments from any type of time series sensor data and can assign semantic labels to any Wi-Fi cluster in human society, such as in hospitals and factories. The authors evaluated the proposed method in real-house environments using leave-one-environment-out cross-validation and achieved state-of-the-art performance despite the unavailability of labeled training data in the target environment.

% \subsubsection{Hybrid}

% \begin{landscape}
% \begin{table}[!th]
% \centering
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c|c
% p{1.1cm}
% p{2cm}
% p{2cm}
% p{1.15cm}
% p{3cm}
% p{3cm}
% p{2cm}
% p{5cm}
% p{1cm}
% p{1.5cm}
% p{4cm}
% p{4cm}
% p{4cm}}
% \hline
% \makecell{Ref.\\ (Year)} & \makecell{Dataset\\Owner} & \# of Datasets & Devices & Sensors & \# of\newline Sensors & Position & Model & \# of Subjects [M/F] & Activities & \# of Activities & \makecell{In-Out\\ Door}& Annotation & Advantages & Limitations \\ \hline \hline
% \cite{szewcyzk2009annotating}&2009&&&&&&&&&&&&&&\\
% \hline \hline
% \end{tabular}}
% \caption{Overview of Semi and Fully-automated methodologies.}\label{tab:SF}
% \end{table}
% \end{landscape}

% \subsubsection{Transfer Learning}
% \blindtext
% \blindtext

% \begin{table}[!h]
% \centering
% \begin{tabular}{c|ccccc}
% \hline \hline
% Ref. & Devices & Activities & \# of Subjects & Collected data & Limitations \\ \hline
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \hline \hline
% \end{tabular}
% \caption{Caption}\label{tab:my_label}
% \end{table}

% \subsubsection{Semantic/Heuristics}
% \blindtext
% \begin{table}[!h]
% \centering
% \begin{tabular}{c|ccccc}
% \hline \hline
% Ref. & Devices & Activities & \# of Subjects & Collected data & Limitations \\ \hline
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \hline \hline
% \end{tabular}
% \caption{Caption}\label{tab:my_label}
% \end{table}
% \blindtext




% \subsection{Human}
% \blindtext
% \subsubsection{One}
% \blindtext
% \blindtext

% \begin{table}[!h]
% \centering
% \begin{tabular}{c|ccccc}
% \hline \hline
% Ref. & Devices & Activities & \# of Subjects & Collected data & Limitations \\ \hline
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \hline \hline
% \end{tabular}
% \caption{Caption}\label{tab:my_label}
% \end{table}

% \subsubsection{Two}
% \blindtext
% \blindtext

% \begin{table}[!h]
% \centering
% \begin{tabular}{c|ccccc}
% \hline \hline
% Ref. & Devices & Activities & \# of Subjects & Collected data & Limitations \\ \hline
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \cite{...}&&&&&\\
% \hline \hline
% \end{tabular}
% \caption{Caption}\label{tab:my_label}
% \end{table}

\subsection{Categorization by used sensing device}\label{sec:4.3}
As can be inferred from the previous sections, sensing devices play a pivotal role in HAR and related data annotation techniques. These devices, ranging from wearable sensors to environmental sensors, enable the collection of essential data that provide insights into individuals' activities and behavior patterns. By accurately capturing information such as motion, location, heart rate, and environmental context, sensing devices serve as the foundation for HAR systems. 

The data collected by these sensing devices serve as the raw material for data annotation techniques in HAR. 
Sensing devices facilitate data annotation techniques in several ways. Firstly, they provide objective and quantitative measurements of various physical and environmental parameters, ensuring the accuracy and reliability of the annotated data. This reliability is essential for developing robust HAR models.
Secondly, sensing devices offer real-time or near real-time data, allowing for immediate feedback and annotation during data collection. This feature is particularly valuable in scenarios where prompt intervention or feedback is necessary, such as monitoring athletic performance or tracking a patient's rehabilitation progress. 

Furthermore, sensing devices allow for the annotation of contextual information, such as the location and environmental conditions during specific activities. This additional contextual data enriches the understanding of human behavior and contributes to more nuanced and comprehensive activity recognition models. 


To underscore the significance of sensing devices, Table \ref{tab:category} offers a comprehensive overview of the various sensing devices and associated sensors employed in the methodologies and data annotation techniques explored in the preceding sections. 
\begin{table}[!ht]
\centering
\caption{Categorization of Data Annotation Techniques based on Automation and Data Collection sensor.}\label{tab:category}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c||c|c|c||c|c|c|}
\cline{3-8}
\multicolumn{2}{c}{}&\multicolumn{6}{|c|}{Data annotation techniques in HAR}\\
\cline{3-8}
\multicolumn{2}{c}{}&\multicolumn{3}{|c||}{Semi-automated} &\multicolumn{3}{c|}{Fully-automated} \\ \hline \hline
Sensing Device & Involved Sensors & Data-Centric & Environment & Hybrid & Data-Centric & Environment & Hybrid
% &&based&based&&based&based&\\ \hline
\\
\hline \hline
Video         & Images &
\cite{martindale2018smart} \cite{kwon2020imutube} \cite{avsar2021benchmarking} \cite{korpela2021reducing} &
&
\cite{alam2015mobeacon} \cite{nino2016scalable} & 
\cite{jardim2016automatic} \cite{zhang2020deep} \cite{qi2022dcnn} 
&& \\ \hline
Inertial & \makecell{Accelerometer\\Gyroscope\\ Magnetometer} &

\makecell{
\cite{saeedi2017co} \cite{martindale2018smart} \cite{gan2018automatic} \cite{bota2019semi} \\ 
\cite{martindale2019hidden} \cite{ponnada2019designing} \cite{faridee2019augtoact} \cite{hossain2019active} \\ \cite{sawano2020annotation} \cite{kwon2020imutube} 
\cite{tang2021selfhar} \cite{yhdego2022fall} \cite{mohamed2022har}} &

\cite{subramanya2012recognizing} \cite{woznowski2017talk} \cite{tonkin2018talk} \cite{solis2019human}&

\cite{alam2015mobeacon} \cite{meurisch2015labels}  \cite{cruciani2018automatic} \cite{cruz2019semi} & 

\makecell{\cite{rokni2018autonomous} \cite{liang2018automatic} \cite{zhang2020deep} 
\cite{jeng2021wrist} \\ \cite{ullrich2021detection} \cite{ma2021unsupervised} \cite{qi2022dcnn} \cite{lin2022clustering}} & 

\cite{loseto2013mining} \cite{al2017annotation} \cite{demrozi2021towards} \cite{dissanayake2021indolabel} & 
\\ \hline

Environmental &  \makecell{Pressure\\ Temperature\\ Brightness\\ GPS\\ Microphone\\ PIR} & 
\cite{martindale2018smart} \cite{martindale2019hidden} &
\cite{subramanya2012recognizing} \cite{woznowski2017talk} \cite{tonkin2018talk} & 
\cite{cruciani2018personalized} \cite{meurisch2015labels}  \cite{cruz2019semi}  \cite{tonkin2019towards}& 
& 
\cite{loseto2013mining}\cite{al2017annotation}&
\\ \hline

Physiological &  \makecell{Heart rate\\ Oxygen\\ Blood pressure} &
&
\cite{mohamed2022har} & 
&
& 
&
%\cite{mohamed2022har}
\\ \hline

Radio signals &  \makecell{Bluetooth\\ WiFi}& &
&
\cite{alam2015mobeacon} \cite{meurisch2015labels}&
&
\cite{demrozi2021towards} \cite{dissanayake2021indolabel}&
\\ 
\hline
\hline
\end{tabular}}
\end{table}
By providing a structured representation of the devices and sensors used, the table highlights their crucial role in capturing and annotating data in the defined annotation categories. 
Empirical evidence demonstrates that among the different sensing devices employed, inertial sensors have emerged as the most widely utilized for data collection and annotation purposes. Inertial sensors, which encompass accelerometers, gyroscopes, and magnetometers, offer the ability to measure and record an individual's motion, orientation, and spatial positioning. Their popularity can be attributed to their versatility, portability, and ability to provide real-time and fine-grained data. %In various human activity recognition studies, inertial sensors have been extensively leveraged to capture and annotate data related to activities such as walking, running, cycling, and gestures. 
The inherent advantages of inertial sensors have positioned them as a dominant choice for researchers and practitioners in the field, facilitating accurate and reliable data annotation for a wide range of applications.

